Log Barriers for Safe Black-box Optimization with Application to Safe Reinforcement Learning

Optimizing noisy functions online, when evaluating the objective requires experiments on a deployed system, is a crucial task arising in manufacturing, robotics and many others. Often, constraints on safe inputs are unknown ahead of time, and we only obtain noisy information, indicating how close we are to violating the constraints. Yet, safety must be guaranteed at all times, not only for the final output of the algorithm. We introduce a general approach for seeking a stationary point in high dimensional non-linear stochastic optimization problems in which maintaining safety during learning is crucial. Our approach called LB-SGD is based on applying stochastic gradient descent (SGD) with a carefully chosen adaptive step size to a logarithmic barrier approximation of the original problem. We provide a complete convergence analysis of non-convex, convex, and strongly-convex smooth constrained problems, with first-order and zeroth-order feedback. Our approach yields efficient updates and scales better with dimensionality compared to existing approaches. We empirically compare the sample complexity and the computational cost of our method with existing safe learning approaches. Beyond synthetic benchmarks, we demonstrate the effectiveness of our approach on minimizing constraint violation in policy search tasks in safe reinforcement learning (RL).

==> 8_experiments.tex <==
\clearpage
\section{EXPERIMENTS}
\textcolor{blue}{TODO}
We conduct our experiments on two different practical applications for two different information set-ups described in the paper: 1) zeroth order safe stochastic optimization and 2) first order safe stochastic optimization. We aim to answer the following questions and compare to the following benchmarks:

\begin{itemize}
    \item \emph{Zeroth order optimization for high dimensional task with $d = 40$}: 
    How our proposed zeroth order safe log barrier approach compares to Bayesian safe methods like SafeOpt, Safe LineBO, [Goose](https://las.inf.ethz.ch/files/turchetta19goose-slides.pdf)? We compare them on the parameter tuning task with zero-th order noisy information, in particular on the model constructed based on the SwissFel data (simulator with $d = 2$).
    \item \emph{First order optimization for large dimensional task with $d>>1000$:}
How our proposed algorithm helps for solving the high-dimensional safe Reinforcement Learning (RL) task using the stochastic first-and-zeroth order oracle and compares to the Lagrangian approach? How does it help for fine-tuning of the pre-trained safe policy and model? We run our experiments on [SafetyGym](https://openai.com/blog/safety-gym/) SG6 benchmark as described in [Ray et al. (2019).](https://cdn.openai.com/safexp-short.pdf)
\end{itemize}

\subsection{SwissFel parameters tuning}

In this experiment we use a Gaussian Process based surrogate model constructed using the real data from SwissFel, Switzerland's X-ray free-electron laser at the Paul Scherrer Institute. This model simulates the noisy measurements of the system behaviour dependent on $d=40$ parameters. The main objective is to maximize the pulse energy measured by a gas detector. 

\emph{[Taken from [Johannes' paper]
% (https://www.research-collection.ethz.ch/bitstream/handle/20.500.11850/385955/kirschner19swissfel.pdf?sequence=1&isAllowed=y)
, need to rephrase, but the setup is the following:]}

\emph{Objective:} Per shot pulse energy measured with a gas detector, averaged over 10 measurements at 25-50 Hz. With the settling and computation time, we are able to run 1-2 optimization steps per second.

\emph{Tuning parameters:}
\begin{itemize}
    \item 24 (horizontal \& vertical) beam position monitor (BPM) target values of the orbit feedback through the undulators (maintaining 2 fixed points in each plane).
    \item 5 matching quadrupoles before the undulators.
    \item 11 gap settings of the undulators.
\end{itemize}

\emph{Constraints:}

As a constraint we used a lower bound on the FEL signal. A possible use-case is parasitical tuning during user operation, where a minimum signal is required. Losses were not a major concern with these parameters, but could be included for other parameters or for optimization on other accelerators (e.g. proton accelerators).

The methods we compare with are the methods designed for the safe parameters tuning based on the Bayesian Optimization. 
We measure the following parameters to compare their performance: 
\begin{itemize}
    \item computational complexity (runtime)
    \item sample complexity (number of required measurements)
    \item safety (number of constraint violations)
\end{itemize}


\clearpage

\subsection{ Safe Transfer Learning on Safety Gym}
\paragraph{The safe transfer learning task}
The transfer learning task is in general very important task. For example, given the autonomous driving taxi-car that has a well trained policy working safely for some particular city, one would like to transfer this policy to a new city, that has different specifications. Given that after the direct transfer, the old policy on a new environment still behaves safely but not optimally any more, we would like to improve its performance by collecting the new data using online agent-world interactions. At the same time, we would like to keep all the policy updates during the learning on a safe side, which is extremely important for such tasks as the  autonomous driving in a real city. 
\paragraph{Safety Gym}
We demonstrate the performance of algorithm for safe transfer learning
% on the
% model-based reinforcement learning task 
using the Safety Gym simulator. The Safety Gym has different set-ups: combinations of the agent dynamics and the task setup. For example, the agent \textbf{Point} is described as follows:  A simple robot constrained to the 2D-plane, with one actuator for turning and another for moving forward/backwards. The task \textbf{Goal} means: Move the robot to a series of goal positions. When a goal is achieved, the goal location is randomly reset to someplace new, while keeping the rest of the layout the same. The sparse reward component is attained on achieving a goal position (robot enters the goal circle). The dense reward component gives a bonus for moving towards the goal. For each of the set-ups, there are two levels of complexity. For example, the second complexity level  PointGoal2 stands for larger amount of different obstacles compared to the first one PointGoal1. Our goal is given the safe policy pre-trained using an unsafe algorithm on the simpler environment set-up as a starting policy, to update the policy in such a way that it improves its performance on the harder set-up, with minimum amount of constraint violations during the learning.
% It has an agent moving in some environment, collecting the targets, and avoiding the obstacles. 

% \paragraph{Model-Based Reinforcement Learning} We assume the Markov Chain model with the states $s_t \in S$, possible actions $a_t\in A$, and the stochastic dynamics described by the transition probability $p(s_{t+1}|s_{t}, a_t)$, the goal is to design a stochastic policy of choosing the next action $\pi = p(a_t| s_t)$.

% \paragraph{Markov decision processes}
\paragraph{Constrained Markov decision processes (CMPDs)}
To learn the policy in a model-based manner, we first consider a Markov decision process with the states $\vs_t \in \R^n$ and actions $\va_t \in \R^m$ for $t \in \{0, \dots, T\}$. At each episode we sample from the initial-state distribution $\vs_0 \sim \rho(\vs_0)$, then 
at each step $t$ the agent takes an action by sampling from a policy distribution $\va_t \sim \pi(\cdot | \vs_t)$. 
The next state is then sampled from a transition distribution $\vs_{t + 1} \sim p(\cdot | \vs_t, \va_t)$. The agent observes a reward $r_t \sim p(\cdot | \vs_t, \va_t)$. 
The performance of a pair of policy $\pi$ and dynamics $p$ is defined by
\begin{equation}
    \label{eq:rl-objective}
    J(\pi, p) = \E_{\va_t \sim \pi, \vs_{t + 1} \sim p, \vs_0 \sim \rho} \left[\sum_{t = 0}^{T} r_t \big\rvert \vs_0\right].
\end{equation}


% To make the agent adhere 
% to human-defined safety constraints, we adopt the constrained Markov decision process formalism of \citet{altman-constrainedMDP}.
% In Constrained Markov decision processes , 
% alongside with the reward, 
Additionally, the agent observes cost signals $c_t^i$ 
% generated by $c_t^i \sim p(\cdot | \vs_t, \va_t)$
where $i = 1, \dots, C$. 
% denote the distinct unsafe behaviors we want the agent to avoid. 
For Safety Gym problem, the cost function is  $c(\vs_t) = \1_\mathrm{\vs_t \in \mathcal{H}}$, where $\mathcal{H}$ is the set of harmful states in which an agent hits an obstacle. Given $c_t$, we define the constraint as
\begin{equation}
    \label{eq:cmdp-cons}
    \hat J(\pi, p) = \E_{\va_t \sim \pi, \vs_{t + 1} \sim p, \vs_0 \sim \rho} \left[\sum_{t = 0}^{T} c_t \big\rvert s_0\right] \le d, \;
    % \forall i \in \{1, \dots, C\},
\end{equation}
where $d$ is a human-defined threshold. 
% For example,  
In this case, the constraint  (\ref{eq:cmdp-cons}) can be interpreted as a bound on the probability of visiting the harmful states. We want to find a policy that for the true unknown dynamics $p^\star$ solves 
\begin{equation}
    \label{eq:safe-rl-objective}
    \begin{aligned}
	    \max_{\pi \in  \Pi} &  \; J(\pi, p^\star) \; 
	    \\ \text{s.t. } 
	    & \hat J(\pi, p^\star) \le d. 
	   % \; \forall i \in \{1, \dots, C\}.
    \end{aligned}
\end{equation}

\paragraph{Our model} We base our world model on the Recurrent State Space Model (RSSM) introduced in \citet{hafner2019planet}. The RSSM models the predictive distribution $p(\vs_{\tau:\tau + H} | \vs_{\tau - 1}, \va_{\tau - 1:\tau + H -1}, \theta)$ as a differentiable function, denoted by $p_{\theta}(\vs_{\tau:\tau + H} )$ for simplicity. 
This property allows us to perform the constrained policy optimization by backpropagating gradients through the model. 

For the task and safety critics, we use the reward value function $v(\vs_t)$ and the cost value function of the constraint $\hat v(\vs_t) $.
% \; \forall i \in \{1, \dots, C\}$. 
We model $v(\vs_t)$ and $\hat v(\vs_t)$ as neural networks with parameters $\psi$ and $\psi^i$ respectively. 
% Note that we omit here the dependency of the critics in $\pi$ to reduce the notational clutter.
As in \citet{DBLP:journals/corr/abs-1912-01603}, we use TD$(\lambda)$ \citep{10.5555/3312046}. 
% to trade-off the bias and variance of the critics with bootstrapping and Monte-Carlo value estimation. 
% To learn the task and safety critics, we minimize the following loss function
% \begin{equation}
%     \label{eq:value-loss}
%     \mathcal{L}_{v_\psi^\pi}(\psi) = \E_{\pi, p(\vs_{\tau:\tau + H} | \vs_{\tau - 1}, \va_{\tau - 1:\tau + H -1}, \theta)}\left[\frac{1}{2} \sum_{t = \tau}^{\tau + H} \left(v_\psi^\pi(\vs_t) - \V_\lambda (\vs_t)\right)^2 \right]
% \end{equation}
% which uses the model to generate samples from $p(\vs_{\tau:\tau + H} | \vs_{\tau - 1}, \va_{\tau - 1:\tau + H -1}, \theta)$. 
We denote $v_\psi^\pi$ as the neural network that approximates its corresponding value function and $\V_\lambda$ as the TD$(\lambda)$ value as presented in \citet{DBLP:journals/corr/abs-1912-01603}. Similarly, $\hat \V_\lambda^i$ is the TD($\lambda$) value of the constraint. 
% Note that, while we show here only the loss for the task critic, the loss function for the safety critics is equivalent to \Cref{eq:value-loss}.

We model the policy as a Gaussian distribution via a neural network with parameters $\xi$ such that $\pi_\xi(\va_t | \vs_t) = \mathcal{N}(\va_t; \text{NN}_\xi^\mu(\vs_t), \text{NN}_\xi^\sigma(\vs_t))$. We sample a sequence $\vs_{\tau: \tau + H} \sim p_{\theta}(\vs_{\tau:\tau + H} )$, utilizing $\pi_\xi$ to generate actions on the fly.
% (see \Cref{sec:sequence-sampling}). 
% We approximate $J^i(\pi_\xi)$ in $\varPsi^i(\pi_\xi; \lambda_k^i, \mu_k)$ (recall \Cref{eq:penalty}) as
% \begin{equation}
% \label{eq:constrained-loss-approx}
% 	J^i(\pi_\xi) \approx \E_{\pi_\xi, p(\vs_{\tau:\tau + H} | \vs_{\tau - 1}, \va_{\tau - 1:\tau + H - 1}, \theta)}\left[\sum_{t = \tau}^{\tau + H} \V_\lambda^i(\vs_t)\right].
% \end{equation}
% Moreover, the first expression in the policy's loss (\ref{eq:policy-loss}) approximates $J(\pi_\xi)$. 
We backpropagate through $p_{\theta}(\vs_{\tau:\tau + H} )$ using path-wise gradient estimators \citep{mohamed2020monte}.

% We define a set of statistically plausible transition distributions denoted by $\mathcal{P}$ and let $p_\theta \in \mathcal{P}$ be a particular transition density in this set. Crucially, we assume that the true model $p^\star$ is within the support of $\mathcal{P}$, and that by sampling $\theta \sim p(\theta | \mathcal{D})$ the conditional predictive density satisfies $p(\vs_{t + 1} | \vs_t, \va_t, \theta) = p_\theta \in \mathcal{P}$. These assumptions lead us to the following constrained problem
% \begin{equation}
%     \label{eq:optimism-pessimism}
%         \begin{aligned}
% 	    \max_{\pi \in \Pi} &  \; \max_{p_\theta \in \mathcal{P}} J(\pi, p_\theta)
% 	    & \text{s.t. } \; \max_{p_{\theta^i} \in \mathcal{P}} J^i(\pi, p_{\theta^i}) \le d^i, \;  \forall i \in \{1, \dots, C\}.
%     \end{aligned}
% \end{equation}
 
 By sampling the sequence of states $\{\vs_t\}_{t=\tau}^{\tau+H}$, we approximate the stochastic inexact models of  $J(\pi_\xi), \hat J(\pi_\xi)$ as follows
\begin{align}
\label{eq:constrained-loss-approx}
	& \mathcal J (\pi_\xi| p_{ \theta}, v_{\psi}) 
% 	\approx \E_{\pi_\xi, p_\theta, v_{\psi}}
	= \left[\sum_{t = \tau}^{\tau + H} \V_\lambda(\vs_t)\right]\\
	& \hat {\mathcal J}(\pi_\xi| p_{\hat\theta}, v_{\hat \psi}) 
% 	\approx \E_{\pi_\xi, p_\theta, v_{\hat \psi}}
	= \left[\sum_{t = \tau}^{\tau + H}\hat \V_{ \lambda}( \vs_t)\right].
\end{align}
 We also get the gradients of the above stochastic functions over $\xi$ using the backpropagation. Therefore, we assume the stochastic first-order oracle.
 
%  Finally, we approximate it with the following constrained problem
% \begin{equation}
%     \label{eq:optimism-pessimism}
%         \begin{aligned}
% 	    \max_{\xi} &  \; \max_{p_\theta \in \mathcal{P}} J(\pi_{\xi}, p_\theta)
% 	    & \text{s.t. } \; \max_{p_{\hat \theta} \in \mathcal{P}} \hat J(\pi_{\xi}, p_{\theta^i}) \le d, 
% 	   % \;  \forall i \in \{1, \dots, C\}.
%     \end{aligned}
% \end{equation}
% \paragraph{Model Based Reinforcement Learning}
% That is, we build Neural Network(NN) based models of:
% \begin{itemize}
%     \item the policy $\pi_{\theta}$, the NN simulates the mean and the variance of $a_t$ given $s_t$ for a Gaussian distribution.
%     \item the dynamics described by the transition probability $p(s_{t+1}|s_{t}, a_t) \sim$  NN($\phi$), NN simulates the mean and the varince of the upcoming state $s_{t+1}$ for a Gaussian distribution.
%     \item the critics of the objective value function $v_{\psi}$ (describing the prediction of the discounted sum of rewards) and of the constraint value function for each of the constraints $v^i_{\psi^i}$(analogously).
% \end{itemize}



% These models allow us to assume that at each iteration we have an inexact model of the objective $J(\pi_{\theta})$ and of the constraints $J^i(\pi_{\theta}) \forall i = 1,\ldots,m$ for the problem, formulated by

% \begin{align} 
%     &\max_{\pi \in \Pi}   \; J(\pi) \\
%     &\text{s.t. } J^i(\pi) \le d^i, \; \forall i \in \{1,\ldots,m\}
% \end{align}

% We consider the constrains given as a potential number of hitting an obstacle in the future. We can build a non-parametric high probability upper bound on it by sampling several posterior trajectories and taking the least safe trajectory among them to estimate the constraint gradient of $\nabla J^i(\pi_{\theta})$. 

% Crucially, we assume that the true model $p^\star$ is within the support of $\mathcal{P}$, and that by sampling $\theta \sim p(\theta | \mathcal{D})$ the conditional predictive density satisfies $p(\vs_{t + 1} | \vs_t, \va_t, \theta) = p_\theta \in \mathcal{P}$. These assumptions lead us to the following constrained problem
% \begin{equation}
%     \label{eq:optimism-pessimism}
%         \begin{aligned}
% 	    \max_{\pi \in \Pi} &  \; \max_{p_\theta \in \mathcal{P}} J(\pi, p_\theta)
% 	    & \text{s.t. } \; \max_{p_{\theta^i} \in \mathcal{P}} J^i(\pi, p_{\theta^i}) \le d^i, \;  \forall i \in \{1, \dots, C\}.
%     \end{aligned}
% \end{equation}

\paragraph{Experimental setup} In all our experiments, the agent observes 64$\times$64 pixels RGB images, taken from the robot's point-of-view. 
% Also, since there is only one safety constraint, we let $J_c(\pi) \equiv J^1(\pi)$.
We measure performance with the following metrics, as proposed in \citet{Ray2019}:
\begin{itemize}
	\item Average undiscounted episodic return for $E$ episodes: $\bar{J}(\pi) = \frac{1}{E} \sum_{i = 1}^{E} \sum_{t = 0}^{T_{\text{ep}}} r_t$
	\item Average undiscounted episodic cost return for $E$ episodes: $\bar{J}_c(\pi) = \frac{1}{E} \sum_{i = 1}^{E} \sum_{t = 0}^{T_\text{ep}} c_t$
	\item Normalized sum of costs during training, namely the \emph{cost regret}: for a given number of total interaction steps $T$, we define $\rho_c(\pi) = \frac{\sum_{t = 0}^{T} c_t}{T}$ as the cost regret.
\end{itemize}
We compute $\bar{J}(\pi)$ and $\bar{J}_c(\pi)$ by averaging the sum of costs and rewards across $E = 10$ evaluation episodes of length $T_{\text{ep}} = 1000$, without updating the agent's networks and discarding the interactions made during evaluation. In contrast to the other metrics, to compute $\rho_c(\pi)$, we sum the costs accumulated {\em during training} and not evaluation episodes.

For the first 1M steps we train the policy and the models using the LAMBDA algorithm on the SafetyGym environment PointGoal1. Then, we switch the environment to a harder one PointGoal2, and for the second 1M steps starting from the previously obtained policy, we continue training it with the Log Barrier algorithm. We compare its performance with the setup when we continue training on the second stage with the LAMBDA algorithm. 


% Also, we check how it behaves 
% The results for all methods are recorded once the agent reached 1M environment steps for PointGoal1, PointGoal2, CarGoal1 and 2M steps for PointButton1, PointPush2, DoggoGoal1 environments respectively. To reproduce the scores of TRPO-Lagrangian, PPO-Lagrangian and CPO, we follow the experimental protocol of \citet{Ray2019}. We give further details on our experiment with CEM-MPC at the ablation study section.


% WHICH EXPERIMENT WE ARE MOST INTERESTED:
% \begin{itemize}
% \item tune one more parameter - discount factor for the value function TD$\lambda$.
% ( point goal 2 only before)
% \item try first  pretrain, and then fine-tune using the log barriers
% \item try first to train for one environment (PG1), and then fine tune for another(PG2)
% \item try the new safety control gym 
% \item To use the offline data to train the model, then do the actor-critic part offline as well. us the to have the safe exploration.  Generate the safe dataset manually too, to have the safe events as well, and to train the actor critic safely.
% \end{itemize}

% Then, to learn the policy we use the gradient based methods compare two different approaches:

% \paragraph{Augmented Lagrangian based approach (Explored with Yarden):}
% \begin{itemize}
%     \item it efficiently learns a policy which has a good safety performance (after learning)
%     \item it learns much faster than the model-free RL methods
%     \item its safety during the learning is not the best compared to model-free approaches
%     \item can we improve it by our method?
% \end{itemize}
% We compare the performances of these methods by measuring their:
% \begin{itemize}
%     \item sample complexity
%     \item safety after the learning
%     \item safety during the learning
% \end{itemize}

% \footnote{Compared to the former safe step size based on the Lipschitz constants $L$, the new approach is less conservative since it takes into account the current gradient norm of the constraint, but not the uniform upper bound $L$ on the gradients over the whole set.  
% On the synthetic and LQR experiments the new approach requires at least twice fewer measurements.}

% \section{Comparison on the LQR problem.}
% Consider the linear dynamical system:
% $
%     q_{h+1}  = Aq_h + Bu_h
%     $
% and the following Linear Quadratic Regulation (LQR) problem for reaching the target  $q_{\text{target}}$:
% \vspace{-0.2cm}
% \begin{align}
%     \min_{u}~ \;&\frac{1}{H}\sum_{h=1}^H \|q_h - q_{\text{target}}\|_2^2\\
%     \text{s.t. } \; & q_0 = q^{(0)},~ q_{h+1} = Aq_h + Bu_h,\\
%     & q_h \in \mathcal Q
%     ~~~~~~\forall h = 1,\ldots,H \label{hard_contraint}
% \end{align}
% The matrices $A,B$ are unknown. The goal is to learn the open-loop controller $(u_0,\ldots,u_{H-1})$ minimizing the LQR objective while not violating the hard constraints (\ref{hard_contraint}) during the learning. In our case study, we consider $H = 10$,
%     $A = \begin{bmatrix}1 & 0.5 \\ 0 & 1\end{bmatrix},~ B = \begin{bmatrix}0 \\
%     1 \end{bmatrix},$  $\mathcal Q= \{q\in\R^2: \|q\|_2\leq 3,\, \begin{bmatrix}1&1\end{bmatrix}q \leq 3,\, \begin{bmatrix}-1&-1\end{bmatrix}q\leq 3 \}$, $q_{\text{target}} = [2.5,0],$ $q_0 = [-2,0].$  The input sequence is initialized to $u_h = 0$, $h=0, \dots, H$. Note that for zero input, the trajectory is stationary and therefore safe, since $q_{h+1} = Aq_h = \begin{bmatrix}1 & 0.5 \\ 0 & 1\end{bmatrix}\begin{bmatrix}-2\\ 0\end{bmatrix} = \begin{bmatrix}-2\\ 0\end{bmatrix}$.
% \begin{center}
% \includegraphics[width = 0.49\textwidth]{Figs/Unknown}
% \includegraphics[width = 0.49\textwidth]{Figs/Unknown-2}
% \end{center}

% \section{Application to Safe Reinforcement Learning}
%     \paragraph{Actor Critic reinforcement learning} In this setup the key concepts are:
%     \begin{itemize}
%         \item The reward $r_{t+1} = r(s_t,a_t)$
%         \item (The actor) The policy $\pi_{\theta}: \mathcal S \times \mathcal A \rightarrow \R^+$ is parametrized by Neural Network (NN) parameters $\theta$. The policy $\pi_{\theta}(a|s)$ is the probability to take action $a$ at the state $s$.
%         \item (The critic) The value function $V_{\omega}: \mathcal S \times \mathcal A \rightarrow \R $ parametrized by NN with parameters $\omega$ (other options like TD, Q-function, etc. are possible.) $$V(s_t) = \E_{a_{j}\sim \pi_{\theta}} \sum_{j=t}^{\infty}r(s_j,a_j), \text{but we estimate it by learning NN parametrized by } \omega: V_{\omega}(s)$$ 
%         Then we use the Advantage function as a critic: $A(s_t,a_t) = r_{t+1} + \gamma V_{\omega}(s_{t+1}) -  V_{\omega}(s_{t})$
        
%         (To learn the policy $\theta$) It's gradient $\nabla_{\theta}J(\theta) = \E_{\pi_{\theta}} \sum_{t=1}^{\infty} \nabla_{\theta}\log \pi_{\theta}(a_t|s_t) A(s_t, a_t).$
%         \end{itemize}
%          Consider the problem:
%                 \begin{align*}
%                     \min_{\theta}~ & J(\theta)\\
%                     \text{s.t. } & V_c^i(\theta) \geq 0
%                 \end{align*}
%     \begin{itemize}
%         \item The objective $J(\theta) = \E_{\pi_{\theta}} \sum_{t=1}^{\infty} r_t$ 
%         \item The constraints $c^i(\theta) = dist^i(s_t(\theta)|s_0)= dist^i(\pi_{\theta}(s_{t-1}))$ are for example the smallest distances to the obstacles along the time horizon and the value function $$V^c_{\nu}(s_t):\approx\E_{a_j\sim\pi_{\theta}}\sum_{j = t}^{+\infty}c(s_j,a_j) $$
        
%         \item Robust policy $\pi_{\theta^0}(a,s)$: has to guarantee the satisfaction of the state constraints with high probability $\Prob\{c(s_t) \leq 0\}\geq 1-\de.$ Due to the initial uncertainty of the model, is quite conservative.
%         \end{itemize}
%         \textbf{ Our goal:}  assume we already have a pre-trained $\pi_{\theta^0}(a_t|s_t)$, and a pre-trained $V_{\omega^0}(s_t).$ Now we want to fine-tune it, i.e., find better $\hat \theta$ and $\hat \omega$, but evaluating safe experiments in real world, i.e., under the safe data collection.\\
%          For this fine-tuning task finding the local optimum might be enough. (Transfer learning. The data distribution changed, but not too much. Robust policy is still safe.)
%             % \item The question is: should we use the critic here, and how?
%     All of the  $J(\theta), c^i(\theta)$ are non-linear and unknown, we are somehow close to the optimum, the model exists but locally is not so good.  That is why we propose to use for fine tuning our local model-free black-box safe optimization algorithm. 
%     We can estimate the gradient of $J(\theta)$. We can use this gradient without the estimated  \textcolor{red}{Q.} Can we also estimate the gradients of $c(\theta)? $ Can we set as the objective the model estimation?

%     \paragraph{Fine tuning of robust RL} Still, the Robust RL provides us some policy $\pi_{\theta^0}.$ Sebastian et al. use actor-critic mechanism to train their policy. They train their critic via $Q$-iteration (Perolat et al., 2015; Antos et al., 2008) and then differentiate through the critic using pathwise gradients (Mohamed et al., 2019; Silver et al., 2014) using stochastic gradient ascent for the agent. The our goal is to improve this policy safely using the new real-world data, i.e., starting from the safe policy $\theta^0$, solve the following problem safely
%             \begin{align*}
%                     \min_{\theta}~ & J(\theta)\\
%                     \text{s.t. } & V_c^i(\theta) \geq 0
%                 \end{align*}
%     We already have inexact models of $Q$ and $c?$, and now we compute the stochastic gradients of them by measuring the reward $J(\theta)$, the constraints $V_c^i(\theta)$. The constraint function might be learned value function parametrized by NN. 
    
%     %(e.g. in the pendulum example, Cheetah, etc.).
%     \textcolor{red}{Q.} How to measure them? How to measure their gradients? Or just estimate for zero-th order estimates? Ok, we can run the policy $\pi_{\theta_t}$ for the time horizon $H$ starting from the state $s_{t-1}$ where we stopped last time? Then we can measure the reward for this horizon $H$. Episodic reward? Or always starting from the same starting position?   
    
%     Then, when changing the $\theta_t\rightarrow \theta_{t+1}$ the reward will change, but we will measure it with noise. For example, the starting position is included to this noise. The question then, how how to improve in average, not violation constraints with high probability. E.g., $c(\theta)$ is the sum of violations for the horizon $H$, it is random dependent on the starting position, but this randomness should not influence too much, should be sub-Gaussian (or bounded)... E.g, if we assume that at every time horizon we have to avoid some obstacles and dangerous situations (to me more or less uniform), and how far are we from the obstacles in average depends directly on how safe our algorithm is. We need to have Lipschitz continuity on $\theta.$  
    
%   The Lipschitz continuity assumption is mild and has been used in non-robust model-based RL, see, e.g., Curi et al. (2020a)
%   \textcolor{blue}{[ Curi, S., Berkenkamp, F., and Krause, A. Efficient model-based reinforcement learning through optimistic policy search and planning.]}, where
%  it is noted that neural networks with Lipschitz-continuous
% non-linearities (or GPs with Lipschitz continuous kernels) output Lipschitz-continuous predictions.


% Can we guarantee a smoothness constant for $c^i(\theta)$? Assume that the $c^i$ is a distance to the obstacle, and for time horizon 5 we want it not not to be violated.. And the second long time horizon value constraint $V_c$ that is $c^i(\theta) = dist^i(s_t(\theta)|s_0)= dist^i(\pi_{\theta}(s_{t-1}))$
%  \begin{align*}
%     \min_{\theta}~ & J(\theta)\\
%     \text{s.t. } & V_c^i(\theta) \geq 0
% \end{align*}
                
        

==> Ex_paper/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
% \usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
% \newsiamremark{remark}{Remark}
% \newsiamremark{hypothesis}{Hypothesis}
% \crefname{hypothesis}{Hypothesis}{Hypotheses}
% \newsiamthm{claim}{Claim}

% \title{Log barriers for safe non-convex black-box optimization.}



% Sets running headers as well as PDF title and authors
% \headers{An Example Article}{D. Doe, P. T. Frank, and J. E. Smith}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Log barriers for safe black-box optimization\thanks{Submitted to the editors DATE.
\funding{We thank the support of Swiss 
National Science Foundation, under the grant SNSF 200021\_172781, and ERC under the European Union's Horizon 2020 research and innovation programme 
grant agreement No 815943.}}}

% Authors: full names plus addresses.

\author{
Ilnura Usmanova
\thanks{
Automatic Control Laboratory, ETH Zürich, (\email{ilnurau@control.ee.ethz.ch} %,\url{http://www.imag.com/\string~ddoe/}
).
}
\and Andreas Krause
\thanks{
Machine Learning Institute, ETH Zürich,
 (\email{krausea@ethz.ch})
 }
\and Maryam Kamgarpour
\thanks{
Automatic Control Laboratory, ETH Zürich ,
(\email{mkamgar@control.ee.ethz.ch})
}
%  \footnotemark[3]
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> intro.tex <==
\section{Introduction}
    Many optimization tasks in robotics, manufacturing, health sciences, and finance require minimizing a loss function under constraints and uncertainties. 
    
    Importantly, often these constraints are unknown at the outset of optimization, and one can infer the feasibility of inputs only from noisy measurements.
    %%%%%%%
    Moreover, during the optimization process in the real world, in many applications, it is crucial to only query points that satisfy the constraints, i.e., lie inside the feasible set, since querying infeasible points could lead to tangible harmful consequences \citep{kirschner2019adaptive,7487170}. In the machine learning community, this problem is known as the \emph{safe learning} task. 
    
    In this work, we consider two general information cases.
    When we can only access the objective and constraints from noisy value measurements, we say we consider the black-box (zeroth-order) noisy information setting. In some cases, noisy gradient measurements are also available; in these cases, we say we consider the first-order noisy information setting. We address the safe learning task in both these information settings in our work.
    
    We are not aware of any works addressing the \emph{safe} learning with noisy first-order feedback. But there exists a large body of work aiming to solve this challenge in the black-box information case,
    % Safe optimization in the zeroth- and first-order noisy information setting is challenging because it requires 
    % /
    % In this work, we propose a method for safe optimization in the zero and first-order noisy information setting.
    % There exists a large body of work aiming to solve this problem in the black-box information case
    with most methods based on constrained Bayesian Optimization (BO) \citep{pmlr-v37-sui15,berkenkamp2020bayesian}. Although safe BO algorithms are generally provably safe and globally optimal, without simplifying assumptions,  BO methods suffer from \emph{the curse of dimensionality} \citep{https://doi.org/10.48550/arxiv.1807.02811,https://doi.org/10.48550/arxiv.1902.10675,https://doi.org/10.48550/arxiv.2103.00349}. 
That is, their sample complexity might depend exponentially on the dimensionality of most of the commonly used kernels, including the squared exponential kernel \citep{srinivas12information}. 
	Moreover, their computational complexity can also scale exponentially on the dimensionality since BO methods have to solve a Non-Linear Programming (NLP) sub-problem at each iteration, which is, in general, an NP-hard problem. 
	Together with this challenge, their computational complexity scales cubically with the number of observations, which provides a significant additional restriction on the number of observations.
	These challenges make BO methods harder to employ on medium-to-big scale problems. \footnote{Few works are extending BO approaches to high dimensions, see  \citet{https://doi.org/10.48550/arxiv.1502.05700,kirschner2019adaptive}.}
	
    Thus, the primary motivation behind this work is to find an algorithm such that
    1) its computational complexity  scales  efficiently to a large number of data points;
    2) its sample complexity scales efficiently to high dimensions, and;
    3) it keeps optimization iterates within the feasible set of parameters with high probability. 
    We propose Log Barriers SGD
    % Stochastic Gradient Descent
    (\LBM), an algorithm that addresses the safe learning task by minimizing the log barrier approximation of the problem by using the Stochastic Gradient Descent (SGD) with a carefully chosen adaptive step size. We provide convergence rates for the convex and non-convex case (to the stationary point) and demonstrate \LBM's performance compared to other safe BO optimization algorithms on a series of experiments with various scales. 
     
    \paragraph{Past work}
    Perhaps surprisingly, the field is still not fully explored. There is little prior work addressing safe learning  
    % in the \emph{convex} or \emph{non-convex} setting 
    with \emph{unknown} non-linear constraints in zeroth-order optimization,
     i.e., safe Bayesian approaches \citep{sui2015safe, berkenkamp2016bayesian,kirschner2019adaptive} or safe approaches based on Frank-Wolfe \citep{usmanova2019safe, fereydounian2020safe}. 
     Moreover, despite the first-order stochastic optimization is widely explored \citep{Nemirovsky_Yudin, juditsky:hal-00853911,
    %  Nemirovski_Juditsky_Lan_Shapiro, DVURECHENSKY2021100015,
     Lan_book},  we are not aware of any work addressing \emph{safe} learning for first-order stochastic optimization. 
    Therefore, even though our work also covers the first-order information case, we focus our review on the zeroth-order (black-box, or bandit) optimization.
    
    Most relevant to our work are two areas: 1) \emph{feasible} optimization approaches addressing smooth problems with {\em known} constraints; 2) existing \emph{safe} approaches addressing smooth 
    % {\em non-convex} 
    \emph{unknown} objectives and constraints (including {\em linear} constraints).  Here, by \emph{unknown} constraints, we mean that we only have access to a noisy zeroth-order oracle of the constraints while solving the constrained optimization problem. By feasible optimization approaches, we call all constrained optimization methods that generate a feasible optimization trajectory. For example, dual approaches such as Augmented Lagrangian are infeasible approaches, whereas Projected Gradient Descent and Frank-Wolfe are feasible approaches. 
	
	\paragraph{Known constraints} 
	\looseness=-1 
	We start with smooth 
    bandit optimization with {\em known} constraints. 
    For \emph{convex} problems, \citet{flaxman2005online} propose an algorithm achieving a sample complexity of $ O(\frac{d^2}{\e^4})$ using projections. \citet{bach2016highly} achieve $O\left(\frac{d^2}{\e^3}\right)$ sample complexity for smooth convex problems, and $O\left(\frac{d^2}{\mu\e^2}\right)$ for smooth $\mu$-strongly-convex problems. 
    Since the projections might be computationally expensive, in the projection-free setting, \cite{chen2019projection} propose an algorithm achieving 
    % regret bound $O(dT^{4/5})$ corresponding to 
    a sample complexity of $O(\frac{d^5}{\e^5})$ for stochastic optimization. 
    \citet{garber2020improved} improve the 
    % regret
    bound for projection-free methods to 
    % $O(dT^{3/4}),$ i.e.,
    $ O(\frac{d^4}{\e^4})$ sample complexity. Instead of projections, they require solving Linear Programming (LP) sub-problems at each iteration. 
    \citet{bubeck2017kernel} propose a kernel-based method for adversarial learning achieving  $O(d^{9.5}T^{1/2})$ regret, 
    and conjecture that a modified version of their algorithm can achieve $O(\frac{d^3}{\e^2})$ sample complexity for stochastic black-box convex optimization. This method is quite complicated and at each iteration $t>0$ requires sampling from a specific distribution $p_t$, that can be done in $\text{poly}(d,\log(T))T$-time. 
% 	For the smooth and convex case, \citet{belloni2015escaping} propose the method that achieves $O(\frac{d^{6.5}}{\e^2})$.
	For the smooth and strongly-convex case, \citet{hazan2016variance} propose a method that achieves $O(\frac{d^3}{\e^2}).$ The general lower bound for the convex black-box stochastic optimization $O\left(\frac{d^{2}}{\e^2}\right)$ is proposed by \citet{shamir2013complexity}. 
	Up to our knowledge, there is no proposed lower bound for the safe black-box optimization with unknown constraints.
% 	\textit{Lower bound in the unconstrained non-safe case.} 
% In a well-known model where algorithms access smooth,  non-convex functions through queries to an unbiased stochastic gradient oracle with bounded variance, 
% 	However, these methods do not guarantee safety under unknown constraints; they assume either known or no constraints. 
	For \emph{non-convex} optimization, \citet{balasubramanian2018zeroth} provide a comprehensive analysis of the performance of several zeroth-order algorithms allowing two-point bandit feedback. However, they also require knowledge of the constraints\footnote{The difference between one-point and two-point feedback is that two-point feedback allows access to the function with the same noise in multiple points, which is a significantly stronger assumption than the one-point feedback \citep{Duchi2015}}.
	
	There exist also other classical derivative-free optimization methods addressing non-convex optimization based on various heuristics. One example is the Nelder-Mead approach, also known as simplex downhill \citep{10.1093/comjnl/7.4.308}. To handle constraints it uses penalty functions \citep{luersen2004}, or barrier functions \citep{NM-barriers}. Another example are various evolutionary algorithms \citep{journals/jgo/StornP97, kennedy95particle, 10.1007/978-3-642-83814-9_6, journals/ec/HansenO01}.
	Nevertheless, all of these approaches are based on heuristics and thus, do not provide the theoretical convergence rate guarantees, maximum the asymptotic convergence. 
% 	As for the lower bound for the non-convex unconstrained case,  \citet{arjevani2019lower} prove that in the worst case, any algorithm requires at least $\e^{-4}$ queries to find an $\e$ stationary point.  
% 	There are some works in zeroth-order 1-point feedback for convex optimization with known constraints, for example \citet{bach2016highly} require $O\left(\frac{d^2}{\eta^3}\right)$ measurements to achieve $\eta$ accuracy in the non-smooth case.
% 	However, the conditional gradient-based algorithm (Frank-Wolfe) of \citet{balasubramanian2018zeroth} for constrained non-convex problems requires global knowledge of the constraint functions since the linear objective must be optimized with respect to these constraints. 
   
    % Safe Bayesian Optimization
    \paragraph{Unknown constraints} 
    \looseness -1 
    There are much fewer works on safe learning for problems with a non-convex objective and \emph{unknown} constraints.
    
    A significant line of work covers objectives and constraints with bounded Reproducing Kernel Hilbert Space (RKHS) norm \citep{sui2015safe, berkenkamp2016bayesian}, based on {\em Bayesian Optimization (BO)}. 
    Also, for \emph{linear} bandits problem \citet{amani2019linear} design a Bayesian algorithm handling the safety constraints. 
    These works build Bayesian models of the constraints and the objective using Gaussian Processes \citep[GP]{10.5555/1162254} and crucially require a suitable GP prior. 
    In contrast, in our work, we {\em do not} use GP models and do not require a prior model for the functions. Still, the fact that we assume smoothness of the functions (and thus the existence of gradients) can be viewed as imposing a prior knowledge on the functions.  
    Additionally, most of these approaches do not scale to high-dimensional problems. However, \citet{kirschner2019adaptive} proposes an adaptation to higher dimensions using line search called LineBO, which demonstrates very high performance in safe and non-safe learning in practical applications.
    However, they prove the convergence rate theoretically only for the unconstrained case and prove only safety (without convergence) for the constrained case. 
    We compare our approach with their method in high dimensions empirically and demonstrate that our approach can solve the problems in the cases when LineBO struggles.
    
    From the optimization point of view, in the case of \emph{unknown} constraints, projection-based techniques or  Frank-Wolfe-based are not valid without assuming a model of the constraint set since such approaches require solving subproblems with respect to the constraint set. 
    One can build such a model in the special case of polytopic constraints. For example, \citet{usmanova2019safe} proposes a safe algorithm for convex learning with smooth objective and \textit{linear} constraints based on the Frank-Wolfe algorithm. Building on the above, \cite{fereydounian2020safe} propose an algorithm for both convex and non-convex objective and \textit{linear} constraints. Both these methods consider first-order noisy objective oracle and zeroth-order noisy constraints oracle. 
    
	For the more general case of non-linear programming,  \citet{usmanova2020safe} proposes using the log barrier gradient-based algorithm for the non-convex non-smooth problem with the zeroth-order information, showing their sample complexity to be $\tilde O\left(\frac{d^{3}}{\e^9}\right)$, there $\e$ is the target accuracy, and $d$ is the dimensionality of the problem. Here, under $\tilde O(\cdot)$, we hide a multiplicative logarithmic factor. 
	This work is built on the idea of \citep{hinder2019poly} who propose the analysis of the gradient-based approach to solving the log barrier optimization (in the deterministic case).
% 	\citet{hinder2019poly} analyze the trust region method in application to the logarithmic barrier independently of the problem and additionally analyze the gradient descent based approach to solving the log barrier optimization (in the deterministic case).  
	In the current paper, we extend the above works to smooth non-convex ($ \tilde O(\frac{d^2}{\e^7})$), convex ($\tilde O(\frac{d^2}{\e^6})$) and strongly-convex ($\tilde O(\frac{d^2}{\e^5})$) problems for both first-order and zeroth-order stochastic information and provide the improved bounds. 
	Note that the log barrier approach is a special case of the Interior Point Method (IPM). IPM is a feasible optimization approach by definition. 
    By using self-concordance properties of specifically chosen barriers and second-order information,  IPM is highly efficient in solving Linear Programming (LP), Quadratic Programming (QP), and conic optimization problems.
	However, building the barrier with self-concordance properties is not possible for the unknown constraints. Therefore, we focus on particularly the logarithmic barriers.
	
	To finalize, compared to state-of-the-art works with tractable algorithms and known constraints \citep{bach2016highly}, we pay a price of an order $\tilde O(\e^{-3})$ in bandit optimization just for the \emph{safety} with respect to unknown constraints both in convex and strongly-convex cases. In the non-convex  case, we pay $ O(d\e^{-3})$ both for safety and having one-point feedback compared to \citet{balasubramanian2018zeroth} considering $2$-point feedback. As for the computational complexity, our method is projection-free and does not require solving any subproblems compared to the above methods.
    
     We summarize the discussion of the algorithms from the past work  as well as the best known lower bounds 
    in Table \ref{tab:comparison}.
 \paragraph{Our contributions}
	We summarize our contributions  below:
    % The sample complexity is shown in the second column.
% 	\paragraph{Prior work in convex setting } 
    % in a special case of polytopic constraints whose coefficients are rational numbers
    % Safe black-box optimization: liner constraints / non-convex 
% In Table \ref{tab:comparison}, we provide a comparison of our algorithm with the existing ones for unconstrained and constrained convex and non-convex zeroth-order optimization. 
%  In our algorithm, we assume a more realistic and more complicated setup where the noise changes with each measurement. 
% We note that this is the first work that provides the upper complexity bound for the safe algorithm for convex non-linear problems. Deriving the lower bound for this class of problems is an open problem. 
% For a non-convex setup, we could expect \textcolor{red}{in the power of 2 more steps, hence  
% $O\left(\frac{d^2}{\eta^6}\right)$ measurements.
% } 
% 	Non-convex non-smooth problems can be addressed by feasible methods, such as  \citep{topkis1967convergence}, FSQP,
% 	\citep{tang2014feasible}. Another related providing the algorithms for non-convex non-smooth problems is
% 	\citep{facchinei2017feasible}. Unfortunately, all the guarantees are in terms of asymptotical convergence to the stationary point.
% \paragraph{Our Contributions.}
    \begin{itemize}
        \item We propose a unified approach for safe learning given zeroth-order or first-order stochastic oracle. 
         We prove that our approach generates feasible iterations with high probability and converges to a stationary point (or to the optimum in the convex case). 
         Each iteration of the proposed method is computationally cheap and does not require solving any subproblems such as those required for Frank-Wolfe (LP subproblems) or BO-based algorithms (NLP subproblems).
        \item In contrast to the past existing works on the log barrier approach for non-smooth problems \citep{usmanova2020safe}, we develop a less conservative, safe, and adaptive step size dependent on the smoothness constant instead of the Lipschitz constant.
        
        \item We derive the convergence rate of our algorithm for the stochastic non-convex, convex, and strongly-convex problems. We prove the convergence despite the non-smoothness of the log barrier and the increasingly high variance of the log barrier gradient estimator
        \item We empirically show that our method can scale to problems with high dimensions in which previous methods fail.
    \end{itemize}

        
        
\begin{table*}[t]
\scriptsize
\centering
    \begin{tabularx}{\textwidth}{Xcccc}
        % \hline 
        %  \multicolumn{2}{|c||}{\bf Known constraints} & \multicolumn{2}{|c|}{\bf Unknown constraints}
        % \\
        \toprule
          \textbf{Algorithm} & \textbf{Sample complexity} & \textbf{Computational complexity}  & \textbf{Constraints} & \textbf{Convexity}
         \\
       \midrule
         \citet{flaxman2005online} 
         & $O\left(\frac{d^2}{\e^4}\right)$ & projections & known & yes \\
         \midrule
         \citet{bach2016highly} & $O\left(\frac{d^2}{\e^3}\right)$ & projections & known & yes\\
         \midrule
         \citet{bach2016highly} & $O\left(\frac{d^2}{\mu \e^2}\right)$ & projections & known & $\mu$-strongly-convex\\
         \midrule
         \citet{bubeck2017kernel}  
         & $O\left(\frac{d^{3}}{\e^2}\right)$ & samplings from $p_t$ distribution & known & yes \\
        %  \hline \citet{belloni2015escaping} & $O(\frac{d^{6.5}}{\e^2})$ & ? & no & yes & 1-point\\
%          \hline
%          \citet{balasubramanian2018zeroth} & \vtop{
%          \hbox{\strut $O\left(\frac{d}{\e^4}\right)$}
% 		\hbox{\strut \footnotesize 
% 		$O\left(\frac{d}{\e^{3.5}}
% 		\right) + \tilde O \left(\frac{d^4}{\e^{2.5}}
% 		\right) $ }
% 		} & \vtop{
% 		\hbox{\strut
% 		 {gradient steps}}
% 		\hbox{\strut
% 		 {Hessian estimation}}} & no & no & 2-point
% 		 \\
	     \midrule \citet{balasubramanian2018zeroth} &  $O\left(\frac{d}{\e^4%\sqrt[4]{T}
			}\right)$
		 & 
		 $O\left(\frac{1}{\e^2}\right)$ LPs & known & no
		 \\
		 \midrule
         \citet{garber2020improved}
         & $O\left(\frac{d^{4}}{\e^4}\right)$ & $O\left(\frac{1}{\e^2}\right)$ LPs & known & yes 
         \\
         \midrule
          \citet{usmanova2019safe}  
         &  $O\left(\frac{d^{3}}{\e^3}\right)$ & $O\left(\frac{1}{\e^2
			}\right)$ LPs & unknown, linear & yes 
         \\
         \midrule
          \citet{fereydounian2020safe}   
         & $\tilde O\left(\frac{d^{2}}{\e^4}\right)$ & $O\left(\frac{1}{\e^2
			}\right)$ LPs & unknown, linear & yes/no 
         \\
         \midrule
          {\citet{berkenkamp2017safe}}
         & $\tilde O\left(\frac{\gamma(d)}{\e^2}\right)$ & $O\left(\frac{\gamma(d)}{\e^2}\right)$ NLPs & unknown & no 
         \\ 
         \midrule
          {\bf This work }
         & $ O\left(\frac{d^{2}}{\e^7}\right)$ & $\tilde O\left(\frac{1}{\e^3}\right)$ gradient steps & unknown & no 
         \\ 
          \midrule
          {\bf This work }
         & $\tilde O\left(\frac{d^{2}}{\e^6}\right)$ & $\tilde O\left(\frac{1}{\e^2}\right)$ gradient steps & unknown & yes 
         \\ 
         \midrule
          {\bf This work }
         & $\tilde O\left(\frac{d^{2}}{\mu\e^5}\right)$ & $\tilde O\left(\frac{1}{\e^2}\right)$ gradient steps & unknown & $\mu$-strongly-convex 
         \\ 
         \midrule
        {\em Lower bound} \citep{shamir2013complexity} 
      & $O\left(\frac{d^{2}}{\e^2}\right)$ & - &  known & yes 
        % & {\em Lower bound}
        % & unknown 
    %     \\
    %     \midrule
    %     {\em Lower bound} \citep{arjevani2019lower} 
    %   & $O\left(\frac{1}{\e^4}\right)$ & - &  no & no 
        % & {\em Lower bound}
        % & unknown 
        \\
        \bottomrule
    \end{tabularx}
    \caption{Zeroth-order safe smooth optimization algorithms (Bandit Convex Optimization). 
    % \citet{usmanova2019safe} and \citet{fereydounian2020safe} considered setup with smooth objective,  zeroth-order linear constraint oracle and stochastic first-order objective oracle. 
    Many of these works provide the bounds in terms of regret, which can be converted to stochastic optimization accuracy, by dividing the regret by $T,$ and deriving the appropriate $T(\e).$ In the SafeOpt, $\gamma(d)$ depends on the kernel, and might be exponential on $d$. All the above works consider one-point feedback, except for \citet{balasubramanian2018zeroth} who consider 2-point feedback. In \citet{bubeck2017kernel} the sampling can be done in $\text{poly}(d,\log(T))T$-time.}
    \label{tab:comparison}
\end{table*}
\paragraph{Paper organization} In Section \ref{section:problem}, we formalize the problem, define the assumptions and the information setting that we have for the first-order stochastic setting. 
In Section \ref{section:general_approach}, we describe our main approach for solving this problem, describe the main theoretical results that we achieve using this approach, provide the basic algorithm, and prove its safety.
In Section \ref{section:method_specifications}, we describe the method specifications for non-convex, convex and strongly-convex cases. For each of these cases we also provide the suitable optimality criterion and the convergence rate analysis. Then, in Section \ref{section:zeroth-order} we analyse specifically the case of the zeroth-order information, and derive the sample complexity of all specifications of our method in this case. In Section \ref{section:experiments} we compare our approach empirically with other existing safe learning approaches and additionally demonstrate its performance on a large-dimensional RL problem.
% \paragraph{Motivation}this
    % \emph{[TODO]}
    % Problems in which the safe learning is required appear in various areas such as Reinforcement Learning, parameters tuning in manufacturing, robotics, medical trials, and others. In such problems real agent-world interactions are required, and thus, the safety is crucial not to harm the system. We consider two particular examples for the motivation. 
% \paragraph{Safe Reinforcement Learning} 
    % One of important problems is Reinforcement Learning (RL). Consider the autonomous driving task as an example. Firstly, based on the collected dataset in some particular environment, such as a particular city, one trains a safe policy. For example, the Model-Agnostic Meta-Learning \citep{pmlr-v70-finn17a} allows to train a policy that adopts efficiently to any environment. Then, assuming moving to a new environment, we want based on the previous safe policy to adapt it to a new environment. While adaptation, we consider an online real-world interactions with the environment. Therefore, we want to fine-tune the policy in a safe way. Alternatively, we can consider that the initial policy is obtained using the interactions with simulator. Then, we transfer the trained policy to a real world environment in a safe way. Since often the models describing policy are too complex, modeled by deep Neural Networks (NN), we can consider that we only have first and zeroth order information
% \paragraph{Black-box parameters tuning}
    % Consider a real world problem of parameters tuning of a real machine, and the measurements are obtained only by direct measuring. Such problems appear in manufacturing, experiment design, physics, e.g., for example in Swiss Free Electron Laser project. 
% \clearpage

==> keeping_distance.tex <==
                % Consider the function 
% $\sum \frac{1}{-f^i(x_t)} = \sum\frac{1}{\alpha_t^i}.$
% Its gradient then $\eta\sum \frac{\nabla f^i_{\nu_k}(x)}{(-f^i_{\nu_k}(x_t))^2} = \eta\sum \frac{\nabla f^i_{\nu_k}(x)}{(\alpha_t^i)^2}.$

Let us denote the part of the log barrier related to the constraints by:
$$\hat B^{\eta_k}_{\nu_k}(x) = - \eta \sum_{i=1}^m \log (-f^i_{\nu_k}(x)).$$
Then, it's gradient at point $x_t$ is 
$$\nabla \hat B_{\nu_k}^{\eta_k}(x_t) = \eta \sum_{i=1}^m \frac{\nabla f^i_{\nu_k}(x_t)}{ (-f^i_{\nu_k}(x_t))} = \eta \sum_{i=1}^m \frac{\nabla f^i_{\nu_k}(x_t)}{\alpha_t^i}.$$

Note that then
$$g_t = \nabla B^{\eta_k}_{\nu_k}(x_t) + \zeta_t = \nabla f^0(x_t) + \zeta_t  + \nabla \hat B_{\nu_k}^{\eta_k}(x_t).$$ Also, note that $\hat B_{\nu_k}^{\eta_k}(x_t)$ is locally-smooth with $M_2(x_t),$ similarly to $B_{\nu_k}^{\eta_k}(x_t).$ Therefore,

\begin{align*} 
        \hat B_{\nu_k}^{\eta_k}(x_{t+1})
        &
        \leq \hat B_{\nu_k}^{\eta_k}(x_t) - \la \nabla \hat B_{\nu_k}^{\eta_k}(x_t),\gamma_t g_t\ra + \frac{M_{\nu_k}}{2} \gamma_t^2\|g_t\|_2^2 
        \\
        &
        \leq   \hat B_{\nu_k}^{\eta_k}(x_t) - \gamma_t\frac{1}{2}
        \left(
        2
        \la\nabla \hat B^{\eta_k}_{\nu_k}(x_t),
         \nabla \hat B^{\eta_k}_{\nu_k}(x_t) 
         + \nabla f^0_{\nu_k}(x_t) 
         + \zeta_t\ra 
         - 
         \|\nabla \hat B^{\eta_k}_{\nu_k}(x_t) 
         + \nabla f^0_{\nu_k}(x_t) 
         + \zeta_t\|_2^2
         \right)
         \\
    &   =   
         \hat B_{\nu_k}^{\eta_k}(x_t) - \gamma_t\frac{1}{2}
        \left(
        \|\nabla \hat B^{\eta_k}_{\nu_k}(x_t)\|_2^2-
         \|\nabla f^0_{\nu_k}(x_t) 
         + \zeta_t\|_2^2
         \right)
    \end{align*}

Hence, if $\|\nabla \hat B^{\eta_k}_{\nu_k}(x_t)\|_2^2\geq \|\nabla f^0_{\nu_k}(x_t) + \zeta_t\|_2^2,$ 
then $\hat B_{\nu_k}^{\eta_k}(x_{t+1})\leq \hat B_{\nu_k}^{\eta_k}(x_{t})$ starts decreasing. This happens when:
\begin{align}\label{eq:decrease_cond}
    \left\|\sum_{i\in[1,m]}
    \frac{\eta_k \nabla f^i_{\nu_k}(x_t) }{\alpha_t^i}\right\|_2\geq L^0 + \frac{\tau_k}{\eta_k\sqrt{n_k}} \geq \|\nabla f^0_{\nu_k}(x_t) + \zeta_t\|_2 
\end{align}

Note that for any vector $r$, $\|r\|_2 \geq \left\|\la r, \frac{x_t-x_0}{\|x_t-x_0\|_2}\ra \frac{x_t-x_0}{\|x_t-x_0\|_2}\right\|_2 = \la r, \frac{x_t-x_0}{\|x_t-x_0\|_2}\ra.$  Recall that due to convexity 
        $$ \la\nabla f^i_{\nu}(x_t), x_t - x_0\ra \geq f^i_{\nu}(x) - f^i_{\nu}(x_0) \geq \beta - \alpha_t^i \geq \beta/2.$$ Hence, the following holds
\begin{align*}
    \left\|\sum_{i\in[1,m]}
    \frac{\eta_k \nabla f^i_{\nu_k}(x_t) }{\alpha_t^i}\right\|_2 
    & \geq 
    \left\la
    \sum_{i\in[1,m]}
    \frac{\eta_k}{\alpha_t^i} \nabla f^i_{\nu_k}(x_t), \frac{x_t - x_0}{\|x_t - x_0\|_2}
    \right\ra \\
    &
    \geq
    \frac{\eta_k}{R}\sum_{i\in[1,m]}\frac{1}{\alpha_t^i}
     \la\nabla f^i_{\nu_k}(x_t),x_t - x_0\ra \\
     &
     \geq \frac{\beta\eta_k}{2R}
     \sum_{i\in[1,m]}\frac{1}{\alpha_t^i}
    %  \\
    %  &
    %  \geq \frac{\beta\eta_k}{2R}\left(m - \sum_{i=1}^m\log \alpha_t^i\right) TOO ROUGH
\end{align*}
% In the above the last inequality is due to $\log y \geq 1-\frac{1}{y}.$
Thus, the condition
$
% \frac{\beta\eta_k}{2R}\left(m - \sum_{i=1}^m\log \alpha_t^i\right) 
\frac{\beta\eta_k}{2R}
     \sum_{i=1}^m\frac{1}{\alpha_t^i}
\geq L^0 + \tau_k$
this implies (\ref{eq:decrease_cond}). Consequently, 
if 
$$\sum_{i=1}^m\frac{1}{\alpha_t^i} \geq \frac{2R(L^0 + \tau_k)}{\beta\eta_k} = \frac{1}{c\eta_k}.$$
then $\hat B_{\nu_k}^{\eta_k}(x_{t+1}) \leq \hat B_{\nu_k}^{\eta_k}(x_{t}),$ which is by definition:

$$\sum_{i=1}^m \log \alpha^i_{t+1}\geq \sum_{i=1}^m \log \alpha^i_{t}.$$

Can we say that there exists a maximum value for  $\hat B_{\nu_k}^{\eta_k}(x_{t})$? And when it is above, it can only decrease?

Assume that $\hat B_{\nu_k}^{\eta_k}(x_{t}) =  -\sum_{i=1}^m \log \alpha^i_{t} \geq B.$ This implies that each $ \log \frac{1}{\alpha_t^i} 
\geq B - \sum_{-i} \log \frac{1}{\alpha_t^i}.$
can we have some condition on $\sum \frac{1}{\alpha^i}?$

$$\sum \frac{1}{\alpha_t^j} \geq \frac{1}{\alpha_t^i} \geq  e^B \prod_{-i} \alpha_t^j \geq e^B c^{m-1}\eta^{m-1} \approx \frac{1}{c\eta_k}.$$

$$e^B \approx \frac{1}{c^{m} \eta^{m}_k}.$$

$$ B \approx -\log{c^{m} \eta^{m}_k}  \approx -m \log{c \eta_k}.$$

Ok. Assume that by the induction base:
$$\alpha^j_t \leq \frac{z-1}{z} c\eta_k.$$
For the almost active:
$$\frac{z-1}{z}c\eta_k \leq \alpha^j_t \leq  c\eta_k.$$
% And $$\hat B_{\eta_k}^{\nu_k}(x_t) \leq -m\log (c\eta_k)$$
Then, at the next iteration it can happen that:
$\frac{1}{\alpha^j_t} \geq \frac{z-1}{zc\eta_k} $ e.g. for $\prod_{-i} \alpha_t^j \geq (\frac{z-1}{z})^{m-1}\prod_{-i} \alpha_t^j  = \frac{1}{2}\prod_{-i} \alpha_t^j $
\begin{align*}
    & \frac{z-1}{z} = \frac{1}{m^{\frac{1}{m-1}}}\\
    & z-1 = z \frac{1}{2^{\frac{1}{m-1}}}\\
    & z\left(1 - \frac{1}{2^{\frac{1}{m-1}}}\right) = 1\\
    & z = \frac{1}{1 - (0.5)^{\frac{1}{m-1}}}
\end{align*}

Then at the next iteration:
$$ 0.5 \hat B_{\eta_k}^{\nu_k}(x_{t}) \leq \hat B_{\eta_k}^{\nu_k}(x_{t+1}) \leq 2\hat B_{\eta_k}^{\nu_k}(x_{t}).$$

Assume it has increased, it became bigger than $-m\log c \eta$ (but smaller than $-(m-1)\log \frac{z-1}{z} c \eta$). Assume that 

What happens if $\prod_{-i} \alpha_t^j \geq 2$

% $$\log(\alpha_t^i) = \log(\alpha_{t+1}^i) + \frac{1}{2}\frac{\alpha_{t+1}^i -\alpha_{t}^i }{\alpha_{t+1}^i} - \frac{1}{3}\frac{(\Delta \alpha^i_t)^2}{(\alpha_{t+1}^i)^2} + \ldots $$

% $$\log(\alpha_{t+1}^i) = \log(\alpha_{t}^i) + \frac{1}{2}\frac{\alpha_{t}^i -\alpha_{t+1}^i }{\alpha_{t}^i} - \frac{1}{3}\frac{(-\Delta \alpha^i_t)^2}{(\alpha_{t}^i)^2} + \ldots $$


% $$ \sum \log(\alpha_{t}^i) + \frac{1}{2}\frac{\alpha_{t}^i -\alpha_{t+1}^i }{\alpha_{t}^i} \geq  \sum \log \alpha^i_{t+1}\geq  \log \sum \alpha^i_{t} \geq  \sum \log(\alpha_{t+1}^i) + \frac{1}{2}\frac{\alpha_{t+1}^i -\alpha_{t}^i }{\alpha_{t+1}^i} - \frac{1}{3}\frac{(\Delta \alpha^i_t)^2}{(\alpha_{t+1}^i)^2}.$$ 

% $$\sum \frac{\alpha_{t+1}^i}{-\Delta \alpha^i_t} \log (1+\frac{-\Delta \alpha^i_t}{\alpha_{t+1}}) =\sum  \frac{-\Delta \alpha^i_t}{\alpha_{t}^i} \geq 0 $$
% $$\sum \frac{\alpha_{t}^i}{\Delta \alpha^i_t} \log (1 - 1/z) \leq \sum \frac{\alpha_{t}^i}{\Delta \alpha^i_t} \log (1+\frac{\Delta \alpha^i_t}{\alpha_{t}}) \leq 0 $$

% $$ \sum  \frac{1}{2}\frac{\Delta \alpha^i_t }{\alpha_{t+1}^i} - \sum \frac{1}{3}\frac{(\Delta \alpha^i_t)^2}{(\alpha_{t+1}^i)^2} \leq 0 \leq \sum  \frac{1}{2}\frac{\Delta \alpha^i_t }{\alpha_{t}^i}$$
% $$ \sum  \frac{\Delta \alpha^i_t }{\alpha_{t+1}^i} -\frac{\Delta \alpha^i_t }{\alpha_{t}^i} -  \frac{2}{3}\frac{(\Delta \alpha^i_t)^2}{(\alpha_{t+1}^i)^2} \leq 0 $$
% $$ \sum  \frac{-(\Delta \alpha^i_t)^2 }{\alpha_{t+1}^i\alpha_{t}^i}  -  \frac{2}{3}\frac{(\Delta \alpha^i_t)^2}{(\alpha_{t+1}^i)^2} \leq 0 $$
% $$ \sum  \frac{\Delta \alpha^i_t }{\alpha_{t+1}^i} \leq \frac{2}{3}\sum \frac{(\Delta \alpha^i_t)^2}{(\alpha_{t+1}^i)^2} $$

% $$\prod_{i=1}^m\frac{1}{\alpha_{t+1}^i} \geq \prod_{i=1}^m\frac{1}{\alpha_t^i}  $$
% $$\prod_{i=1}^m\frac{\alpha_t^i}{\alpha^i_{t+1}} \leq 1  $$


 
              
% \input{0_outline}
% \input{1_introduction}

==> old_intro.tex <==

% \section{Introduction}
% Many optimization tasks in robotics, manufacturing, health sciences, and finance require minimizing a loss function under constraints and uncertainties. 
%     Optimizing a loss function under partially revealed constraints can be further complicated by the fact that observations are available only inside the feasible set. 
%     %%%%%%%
%     In many of these real-world applications, querying the objective outside the feasibility set leads to tangible consequences that may be hazardous \citep{kirschner2019adaptive,7487170}. In these cases, we also care about \emph{safety} during the optimization process.
%     Crucially, constraints are often unknown upfront, i.e., one can infer the feasibility of inputs only from noisy value measurements. In this case, we say we consider the black-box (zeroth-order) noisy information setting. In the machine learning community, this problem is known as the \emph{safe learning} task. In some cases, noisy gradient measurements are also available; in these cases, we say we consider the first-order noisy information setting.
	
% 	Although we are not aware of any works addressing the safe first-order optimization setting, there exists a large body of work aiming to solve this challenge in the black-box information case.
% 	This work is primarily based on constrained Bayesian Optimization (BO) \citep{pmlr-v37-sui15,berkenkamp2020bayesian}. Safe BO algorithms are generally provably safe and globally optimal. 
% 	However, without assuming sparsity of the objective and constraints, BO methods suffer from \emph{the curse of dimensionality} \citep{https://doi.org/10.48550/arxiv.1807.02811,https://doi.org/10.48550/arxiv.1902.10675,https://doi.org/10.48550/arxiv.2103.00349} That is, their sample complexity might depend exponentially on the dimensionality for most of the commonly used kernels, including the squared exponential kernel \citep{srinivas12information}. 
% 	Moreover, their computational complexity can also scale exponentially on the dimensionality since BO methods have to solve a Non-Linear Programming (NLP) sub-problem at each iteration, which is, in general, an NP-hard problem. 
% 	Together with this challenge, their computational complexity scales cubically with the number of observations, which provides a significant additional restriction on amount of observations.
% 	These challenges make BO methods harder to employ on medium-to-big scale problems. \footnote{Few works are extending BO approaches to high dimensions, see  \citet{https://doi.org/10.48550/arxiv.1502.05700,kirschner2019adaptive}.}

%     Thus, the primary motivation behind this work is to find an algorithm such that
%     1) its computational complexity  scales  efficiently to a large number of data points;
%     2) its sample complexity scales efficiently to high dimensions, and;
%     3) it keeps optimization iterates within the feasible set of parameters with high probability. 
%     We propose Log Barriers SGD
%     % Stochastic Gradient Descent
%     (\LBM), an algorithm that relies on stochastic gradient estimation to solve log barrier optimization sub-problems. We provide convergence rates for the convex and non-convex case (to the stationary point) and demonstrate \LBM's performance compared to other safe BO optimization algorithms on a series of experiments with various scales. 
     
%     \paragraph{Past work}
%     Perhaps surprisingly, the field is still not fully explored. There is a little prior work addressing safe learning  
%     % in the \emph{convex} or \emph{non-convex} setting 
%     with \emph{unknown} non-linear constraints in zeroth-order optimization,
%      i.e., safe Bayesian approaches \citep{sui2015safe, berkenkamp2016bayesian,kirschner2019adaptive} or safe approaches based on Frank-Wolfe \citep{usmanova2019safe, fereydounian2020safe}. 
%      Moreover, despite the first-order stochastic optimization is widely explored \citep{Nemirovsky_Yudin, juditsky:hal-00853911,
%     %  Nemirovski_Juditsky_Lan_Shapiro, DVURECHENSKY2021100015,
%      Lan_book},  we are not aware of any work addressing \emph{safe} learning for first-order stochastic optimization. 
%     Therefore, even though our work also covers the first-order information case, we focus our review on the zeroth-order (black-box, or bandit) optimization. We cover two aspects: 1) \emph{feasible} optimization approaches addressing smooth problems with {\em known} constraints; 2) existing \emph{safe} approaches addressing smooth 
%     % {\em non-convex} 
%     \emph{unknown} objectives and constraints (including {\em linear} constraints).  Here, by \emph{unknown} constraints, we mean that we only have access to a noisy zeroth-order oracle of the constraints while solving the constrained optimization problem. By feasible optimization approaches, we call all constrained optimization methods that generate a feasible optimization trajectory. For example, dual approaches such as Augmented Lagrangian are infeasible approaches, whereas Projected Gradient Descent and Frank-Wolfe are feasible approaches. 
	
% 	\paragraph{Known constraints} 
% 	\looseness=-1 
% 	We start with smooth 
%     bandit optimization with {\em known} constraints. 
%     For \emph{convex} problems, \citet{flaxman2005online} proposes an algorithm achieving a sample complexity of $ O(\frac{d^2}{\e^4})$ using projections. \citet{bach2016highly} achieve $O\left(\frac{d^2}{\e^3}\right)$ sample complexity for smooth convex problems, and $O\left(\frac{d^2}{\mu\e^2}\right)$ for smooth $\mu$-strongly-convex problems. 
%     Since the projections might be computationally expensive, in the projection-free setting, \cite{chen2019projection} proposes an algorithm achieving 
%     % regret bound $O(dT^{4/5})$ corresponding to 
%     a sample complexity of $O(\frac{d^5}{\e^5})$ for stochastic optimization. 
%     \citet{garber2020improved} improve the 
%     % regret
%     bound for projection-free methods to 
%     % $O(dT^{3/4}),$ i.e.,
%     $ O(\frac{d^4}{\e^4})$ sample complexity. Instead of projections, they require solving Linear Programming (LP) sub-problems at each iteration. 
%     \citet{bubeck2017kernel} proposes a kernel-based method for adversarial learning achieving  $O(d^{9.5}T^{1/2})$ regret, 
%     and conjecture that a modified version of their algorithm can achieve $O(\frac{d^3}{\e^2})$ sample complexity for stochastic black-box convex optimization. This method is quite complicated and at each iteration $t>0$ requires sampling from a specific distribution $p_t$, that can be done in $\text{poly}(d,\log(T))T$-time. 
% % 	For the smooth and convex case, \citet{belloni2015escaping} propose the method that achieves $O(\frac{d^{6.5}}{\e^2})$.
% 	For the smooth and strongly-convex case, \citet{hazan2016variance} propose a method that achieves $O(\frac{d^3}{\e^2}).$ The general lower bound for the convex black-box stochastic optimization $O\left(\frac{d^{2}}{\e^2}\right)$ is proposed by \citet{shamir2013complexity}. 
% 	Up to our knowledge, there is no proposed lower bound for the safe black-box optimization with unknown constraints.
% % 	\textit{Lower bound in the unconstrained non-safe case.} 
% % In a well-known model where algorithms access smooth,  non-convex functions through queries to an unbiased stochastic gradient oracle with bounded variance, 

% % 	However, these methods do not guarantee safety under unknown constraints; they assume either known or no constraints. 
% 	For \emph{non-convex} optimization, \citet{balasubramanian2018zeroth} provide a comprehensive analysis of the performance of several zeroth-order algorithms allowing two-point bandit feedback. However, they also require knowledge of the constraints\footnote{The difference between one-point and two-point feedback is that two-point feedback allows access to the function with the same noise in multiple points, which is a significantly stronger assumption than the one-point feedback \citep{Duchi2015}}.
	
% 	There exist also other classical derivative-free optimization methods addressing non-convex optimization based on various heuristics. One example is the Nelder-Mead approach, also known as simplex downhill \citep{10.1093/comjnl/7.4.308}. To handle constraints it uses penalty functions \citep{luersen2004}, or barrier functions \citep{NM-barriers}. Another example are various evolutionary algorithms \citep{journals/jgo/StornP97, kennedy95particle, 10.1007/978-3-642-83814-9_6, journals/ec/HansenO01}.
% 	But all of these approaches are based on heuristics, and thus, do not provide the theoretical convergence rate guarantees, maximum the asymptotic convergence. 
% % 	As for the lower bound for the non-convex unconstrained case,  \citet{arjevani2019lower} prove that in the worst case, any algorithm requires at least $\e^{-4}$ queries to find an $\e$ stationary point.  
% % 	There are some works in zeroth-order 1-point feedback for convex optimization with known constraints, for example \citet{bach2016highly} require $O\left(\frac{d^2}{\eta^3}\right)$ measurements to achieve $\eta$ accuracy in the non-smooth case.
% % 	However, the conditional gradient-based algorithm (Frank-Wolfe) of \citet{balasubramanian2018zeroth} for constrained non-convex problems requires global knowledge of the constraint functions since the linear objective must be optimized with respect to these constraints. 
   
%     % Safe Bayesian Optimization
%     \paragraph{Unknown constraints} 
%     \looseness -1 
%     There are much fewer works on safe learning for problems with a non-convex objective and \emph{unknown} constraints.
    
%     A significant line of work covers objectives and constraints with bounded Reproducing Kernel Hilbert Space (RKHS) norm \citep{sui2015safe, berkenkamp2016bayesian}, based on {\em Bayesian Optimization (BO)}. 
%     Also, for \emph{linear} bandits problem \citet{amani2019linear} designs a Bayesian algorithm handling the safety constraints. 
%     These works build Bayesian models of the constraints and the objective using Gaussian Processes \citep[GP]{10.5555/1162254} and crucially require a suitable GP prior. 
%     In contrast, in our work, we {\em do not} use GP models and do not require a prior model for the functions. Still, the fact that we assume smoothness of the functions (and thus the existence of gradients) can be viewed as imposing a prior knowledge on the functions.  
%     Additionally, most of these approaches do not scale to high-dimensional problems. However, \citet{kirschner2019adaptive} proposes an adaptation to higher dimensions using line search called LineBO, which demonstrates very high performance in safe and non-safe learning in practical applications.
%     However, they prove the convergence rate theoretically only for the unconstrained case and prove only safety (without convergence) for the constrained case. 
%     We compare our approach with their method in high dimensions empirically and demonstrate that our approach can solve the problems in the cases when LineBO struggles.
    
%     From the optimization point of view, in the case of \emph{unknown} constraints projection-based techniques or  Frank-Wolfe-based are not valid without assuming a model of the constraint set since such approaches require solving subproblems with respect to the constraint set. 
%     One can build such a model in the special case of polytopic constraints. For example, \citet{usmanova2019safe} proposes a safe algorithm for convex learning with smooth objective and \textit{linear} constraints based on the Frank-Wolfe algorithm. Building on the above, \cite{fereydounian2020safe} propose an algorithm for both convex and non-convex objective and \textit{linear} constraints. Both these methods consider first-order noisy objective oracle and zeroth-order noisy constraints oracle. 
    
% 	For the more general case of non-linear programming,  \citet{usmanova2020safe} proposes using the log barrier gradient based algorithm to the non-convex non-smooth problem with the zeroth-order information, showing their sample complexity to be $\tilde O\left(\frac{d^{3}}{\e^9}\right)$.  Here, under $\tilde O(\cdot)$, we hide a multiplicative logarithmic factor. 
% 	This work is built on the idea of \citep{hinder2019poly} who propose the analysis of the gradient based approach to solving the log barrier optimization (in the deterministic case).
% % 	\citet{hinder2019poly} analyze the trust region method in application to the logarithmic barrier independently of the problem and additionally analyze the gradient descent based approach to solving the log barrier optimization (in the deterministic case).  
% 	In the current paper, we extend the above works to smooth non-convex ($ \tilde O(\frac{d^2}{\e^7})$), convex ($\tilde O(\frac{d^2}{\e^6})$) and strongly-convex ($\tilde O(\frac{d^2}{\e^5})$) problems for both first-order and zeroth-order stochastic information and provide the improved bounds. 
% 	Note that the log barrier approach is a special case of Interior Point Method (IPM). IPM is a feasible optimization approach by definition. 
%     By using self-concordance properties of specifically chosen barriers and second-order information,  IPM is highly efficient in solving Linear Programming (LP), Quadratic Programming (QP), and Conic optimization problems.
% 	However, building the barrier with self-concordance properties is not possible for the unknown constraints, therefore we focus on particularly the logarithmic barriers.
	
% 	To finalize, compared to state of the art works with tractable algorithms and known constraints \citep{bach2016highly}, we pay a price of an order $\tilde O(\e^{-3})$ in bandit optimization just for the \emph{safety} with respect to unknown constraints both in convex and strongly-convex cases. In the non-convex  case, we pay $ O(d\e^{-3})$ both for safety and having one-point feedback compared to \citet{balasubramanian2018zeroth} considering $2$-point feedback. As for the computational complexity, our method is projection-free and does not require solving any subproblems compared to the above methods.
 
% 	We summarize our contributions  below:
%     \begin{itemize}
%         \item We propose a unified approach for safe learning given zeroth-order or first-order stochastic oracle. 
%          We prove that our approach generates feasible iterations with high probability and converges to a stationary point (or to the optimum in the convex case). 
%          Each iteration of the proposed method is computationally cheap and does not require solving any subproblems such as those required for Frank-Wolfe (LP subproblems) or BO-based algorithms (NLP subproblems).
%         \item In contrast to the past existing works on the log barrier approach for non-smooth problems \citep{usmanova2020safe}, we develop a less conservative, safe, and adaptive step size dependent on the smoothness constant instead of the Lipschitz constant.
        
%         \item We derive the convergence rate of our algorithm for the stochastic non-convex, convex, and strongly-convex problems. We prove the convergence despite the non-smoothness of the log barrier and the increasingly high variance of the log barrier gradient estimator
%         \item We empirically show that our method can scale to problems with high dimensions in which previous methods fail.
%     \end{itemize}
%  We summarize the discussion of the algorithms from the past work  
%     as well as the best known lower bounds 
%     in Table \ref{tab:comparison}.
        


\section{Introduction}\label{section:introduction}	

    Many optimization tasks in robotics, manufacturing, health sciences, and finance require minimizing a loss function under constraints and uncertainties. 
    Optimizing a loss function under partially revealed constraints can be further complicated by the fact that observations are available only inside the feasible set. 
    %%%%%%%
    In many of these real-world applications, querying the objective outside the feasibility set leads to tangible consequences that may possibly be hazardous \citep{kirschner2019adaptive,7487170}. In these cases we also care about \emph{safety} during the optimization process. Crucially, constraints are often unknown upfront, i.e., feasibility of inputs can only be inferred from noisy value measurements, that is, black-box information setting.  In
    the machine learning community, this problem is known as the \emph{safe learning} task. In some cases noisy gradient measurements are also available, that is, it can be a first-order noisy information setting.
	
	Although we are not aware of any works addressing safe first-order optimization setting, there exists a large body of work that aims to solve this challenge in black-box information case. 
	This work is primarily based on constrained Bayesian Optimization (BO) \citep{pmlr-v37-sui15,berkenkamp2020bayesian}. Safe BO algorithms are generally provably safe and globally optimal. 
	However, 
% 	BO commonly relies on Gaussian Processes \citep[GP]{10.5555/1162254}.
	without assuming differentiability or sparsity of the objective and constraints, BO methods suffer from \emph{the curse of dimensionality} \citep{https://doi.org/10.48550/arxiv.1807.02811,https://doi.org/10.48550/arxiv.1902.10675,https://doi.org/10.48550/arxiv.2103.00349}, that is, their sample complexity depends exponentially on the dimensionality. 
	Moreover, their computational complexity also scales exponentially on the dimensionality, since at each iteration BO methods have to solve a Non-Linear Programming (NLP) sub-problem, which is in general an NP-hard problem. 
	Together with this challenge, their computational complexity scales cubically with the number of observations, that provides an additional significant restriction on the number of observations.
	These challenges make BO methods harder to employ on medium-to-big scale problems. \footnote{There are few works extending BO approaches to high dimensions, see  \citet{https://doi.org/10.48550/arxiv.1502.05700,kirschner2019adaptive}.}

    Thus, the main motivation behind this work is to find an algorithm such that
    1) its computational complexity  scales  efficiently to a large number of data-points;
    2) its sample complexity scales efficiently to high dimensions, and;
    3) it keeps optimization iterates within the feasible set of  parameters with high probability. 
We propose Log Barriers SGD (\LBM), an algorithm that relies on zeroth-order gradient estimation to solve log barrier optimization sub-problems. We provide convergence rates for the convex and non-convex case (to the stationary point), and demonstrate \LBM's performance compared to other safe BO optimization algorithms on a series of experiments with various scales. 

	
    % %Motivation
    % Safety is a critical property for many real-world optimization and control problems. Often, safety requirements can be formalized via constraints on the decision variables. However, most work in optimization requires feasibility only for the {\em final output} of the algorithm. When training Reinforcement Learning (RL) agents in simulation, for example, constraint satisfaction is typically not required during training, since evaluating unsafe policies does not harm the simulator. To continue learning in the real world, however, e.g.,  by adaptively fine-tuning solutions obtained from simulations or via first-principle physics models, it becomes important to {\em maintain safety} for all further evaluations during learning. This task is called \textit{safe learning} \citep{sui2015safe, berkenkamp2016bayesian}. Moreover, in such settings, it is often not possible to obtain gradient information and experiments might have noisy outcomes. 
     
    \paragraph{Past work}
    % \textcolor{blue}{add some works on first-order optimization too?}
    Perhaps surprisingly, the field is still not fully explored. There is a little prior work addressing 
    % scalable 
    safe learning  
    % in the \emph{convex} or \emph{non-convex} setting 
    with \emph{unknown} non-linear constraints in zeroth-order optimization,
    % There are few works covering safe learning 
     i.e., safe Bayesian approaches \citep{sui2015safe, berkenkamp2016bayesian,kirschner2019adaptive} or safe approaches based on Frank-Wolfe \citep{usmanova2019safe, fereydounian2020safe}. 
     Moreover, despite the first-order stochastic optimization is widely explored \citep{Nemirovsky_Yudin, juditsky:hal-00853911,
    %  Nemirovski_Juditsky_Lan_Shapiro, DVURECHENSKY2021100015,
     Lan_book},  we are not aware of any work addressing \emph{safe} learning for stochastic first-order optimization. 
    Therefore, despite our work covers also the first-order information case, we focus our review on the zeroth-order (black-box, or bandit) optimization. We cover two aspects: 1) \emph{feasible} optimization approaches addressing smooth problems with {\em known} constraints; 2) existing \emph{safe} approaches addressing smooth 
    % {\em non-convex} 
    \emph{unknown} objectives and constraints (including {\em linear} constraints).  Here, by \emph{unknown} constraints we mean that we only have access to a noisy zeroth-order oracle of the constraints, while solving the constrained optimization problem.  By feasible optimization approaches we call all constrained optimization methods that generate a feasible optimization trajectory. For example, the dual approaches such as Augmented Lagrangian are infeasible approaches, whereas Projected Gradient Descent and Frank-Wolfe are feasible approaches. 
	
	\paragraph{Known constraints} 
	\looseness=-1 
	We start with smooth 
    bandit optimization with {\em known} constraints. 
    For \emph{convex} problems, \citet{flaxman2005online} propose an algorithm achieving a sample complexity of $ O(\frac{d^2}{\e^4})$ using projections. 
    Since the projections might be computationally expensive, in the projection-free setting, \cite{chen2019projection} propose an algorithm achieving regret bound $O(dT^{4/5})$ corresponding to a sample complexity of $O(\frac{d^5}{\e^5})$ for stochastic optimization. 
    \citet{garber2020improved} improve the 
    % regret
    bound for projection-free methods to 
    % $O(dT^{3/4}),$ i.e.,
    $ O(\frac{d^4}{\e^4})$ sample complexity. Instead of projections, they require solving Linear Programming (LP) sub-problems at each iteration. 
    \citet{bubeck2017kernel} propose a kernel-based method for adversarial learning achieving  $O(d^{9.5}T^{1/2})$ regret, 
    and conjecture that a modified version of their algorithm can achieve $O(\frac{d^3}{\e^2})$ sample complexity for stochastic black-box convex optimization. This method at each iteration $t>0$ requires sampling from a specific distribution $p_t$, that can be done in $\text{poly}(d,\log(T))T$-time.
% 	For the smooth and convex case, \citet{belloni2015escaping} propose the method that achieves $O(\frac{d^{6.5}}{\e^2})$.
	For the smooth and strongly-convex case, \citet{hazan2016variance} propose a method that achieves $O(\frac{d^3}{\e^2}).$ The general lower bound for the convex black-box stochastic optimization $O\left(\frac{d^{2}}{\e^2}\right)$ is proposed by  \citet{shamir2013complexity}. 
	Up to our knowledge, there is no proposed lower bound for the safe black-box optimization with unknown constraints.
% 	\textit{Lower bound in the unconstrained non-safe case.} 
% In a well-known model where algorithms access smooth,  non-convex functions through queries to an unbiased stochastic gradient oracle with bounded variance, 

% 	However, these methods do not guarantee safety under unknown constraints, they assume either known constraints, or no constraints at all. 
	For \emph{non-convex} optimization,  \citet{balasubramanian2018zeroth} provide a comprehensive analysis of the performance of several zeroth-order algorithms allowing two-point bandit feedback, however they also require a full knowledge of the constraints\footnote{The difference between one-point and two-point feedback \citep{Duchi2015}}. 
% 	As for the lower bound for the non-convex unconstrained case,  \citet{arjevani2019lower} prove that in the worst case any algorithm requires at least $\e^{-4}$ queries to find an $\e$ stationary point.  
% 	There are some works in zeroth-order 1-point feedback for convex optimization with known constraints, for example \citet{bach2016highly} require $O\left(\frac{d^2}{\eta^3}\right)$ measurements to achieve $\eta$ accuracy in the non-smooth case.
% 	However, the conditional gradient based algorithm (Frank-Wolfe) of \citet{balasubramanian2018zeroth} for constrained non-convex problems requires global knowledge of the constraint functions, since the linear objective must be optimized with respect to these constraints. 
   
    % Safe Bayesian Optimization
    \paragraph{Unknown constraints} 
    \looseness -1 
    There are much fewer works on safe learning for problems with non-convex objective and \emph{unknown} constraints.
    
    A significant line of work covers objectives and constraints with bounded Reproducing Kernel Hilbert Space (RKHS) norm \citep{sui2015safe, berkenkamp2016bayesian}, based on {\em Bayesian Optimization (BO)}. 
     Also, for \emph{linear} bandits problem \citet{amani2019linear} design a Bayesian algorithm handling the safety constraints. 
    These works build Bayesian models of the constraints and the objective using Gaussian Processes \citep[GP]{10.5555/1162254} and crucially require a suitable GP prior. 
    In contrast, in our work we {\em do not} use GP models and  do not require a prior model for the functions. Still, the fact that we assume smoothness of the functions (and thus the existence of gradients) can be viewed as imposing a prior knowledge on the functions.  
    Additionally, most of these approaches do not scale to high dimensional problems. However, \citet{kirschner2019adaptive} propose an adaptation to higher dimensions using line search called LineBO, that demonstrates a very well performance in safe and non-safe learning in practical applications.
    However, they prove theoretically the convergence rate only for the unconstrained case, and prove only safety (without convergence) for the constrained case. 
    We compare empirically our approach with their method in high dimensions, and demonstrate that our approach is capable to solve the problems in the cases when LineBO struggles.
    
    From the black-box optimization point of view, note that in the case of \emph{unknown} constraints, projection-based techniques or  Frank-Wolfe-based are not valid without assuming a model of the constraint set, since such approaches require solving subproblems with respect to the constraint set. 
    In the special case of polytopic constraints one can build such a model, for example, \citet{usmanova2019safe} propose a safe algorithm for convex learning with smooth objective and \textit{linear} constraints based on the Frank-Wolfe algorithm. Building on the above, \cite{fereydounian2020safe} propose an algorithm for both convex and non-convex objective and \textit{linear} constraints. Both of these methods consider first-order noisy objective oracle and zeroth-order noisy constraints oracle. 
    
	The Interior Point Method (IPM) is  a feasible approach by definition, and it is widely used for Linear Programming, Quadratic Programming, and Conic optimization problems. 
	By using self-concordance properties of specifically chosen barriers and second order information, these problems are  shown to be extremely efficiently solved by IPM. 
	However, for the unknown constraints, building the barrier with self-concordance properties is not possible. 
	\citet{hinder2019poly} analyse the trust region method in application to the logarithmic barrier independently on the problem, and additionally analyse the gradient descent based approach to solve the log barrier optimization (in the deterministic case). 
	\citet{usmanova2020safe} extends this gradient log barrier based algorithm to the zeroth-order information case for the non-convex non-smooth problem with non-linear constraints, with sample complexity $\tilde O\left(\frac{d^{3}}{\e^9}\right)$.  Here under $\tilde O(\cdot)$ we hide a multiplicative logarithmic factor. In the current paper, we extend the above work to smooth non-convex, convex and strongly-convex problems for both first-order and zeroth-order stochastic information, and provide the improved bounds. We summarize our contributions  below:
% 	\paragraph{Prior work in convex setting } 
    % in a special case of polytopic constraints whose coefficients are rational numbers
    % Safe black-box optimization: liner constraints / non-convex 
% In Table \ref{tab:comparison}, we provide a comparison of our algorithm with the existing ones for unconstrained and constrained convex and non-convex  zeroth-order optimization. 
%  In our algorithm we assume a more realistic and more complicated setup where the noise is changing with each measurement. 
% We note that this is the first work that provides the upper complexity bound for the safe algorithm for convex non-linear problems. Deriving the lower bound for this class of problems is an open problem. 
% For a non-convex setup we could expect \textcolor{red}{in the power of 2 more steps, hence  
% $O\left(\frac{d^2}{\eta^6}\right)$ measurements.
% } 
% 	Non-convex nonsmooth problems can be addressed by feasible methods, such as  \citep{topkis1967convergence}, FSQP,
% 	\citep{tang2014feasible}. Another related providing the algorithms for non-convex non-smooth problems is
% 	\citep{facchinei2017feasible}. Unfortunately, all the guarantees are in terms of asymptotical convergence to the stationary point.
% \paragraph{Our Contributions.}
    \begin{itemize}
        \item We propose a unified approach for safe learning given zeroth-order or first-order stochastic oracle. 
         We prove that our approach generates feasible iterations  with high probability, and prove its convergence  to a stationary point (or to the optimum in the convex case). 
         Each iteration of the proposed method is computationally cheap and does not require solving any subproblems such as those required for Frank-Wolfe (LP subproblems) or Bayesian Optimization based algorithms (NLP subproblems).
        \item In contrast to the past existing works on the log barrier approach for non-smooth problems \citep{usmanova2020safe}, we develop a less conservative safe, and adaptive step size dependent on the smoothness constant instead of the Lipschitz constant.
        % , in contrast to the previous work.
        
        \item We derive the convergence rate of our algorithm for the stochastic non-convex, convex, and strongly-convex problems. We prove the convergence despite the non-smoothness of the log barrier and the increasingly high variance of the log barrier gradient estimator
        \item We empirically show that our method is capable of scaling to problems with high dimensions in which previous methods fail.
    \end{itemize}
 We summarize the discussion of the algorithms from the past work  
    as well as the best known lower bounds 
    in Table \ref{tab:comparison}.

==> proofs.tex <==
\appendix
\section{Proofs}
\subsection{Proof of Lemma \ref{lemma:LBGradEstimatorVarBias}}
\subsubsection{Bias}\label{appendix:bias}
\begin{proof}
    Using $\E[XY]\leq \sqrt{\E [X^2] \E [Y^2]}$, we get
    \begin{align*}%\label{bias_lb}
        \|b_t\|
         & = 
        \|\E[g_t - \nabla B_{\eta}(x_t)|\mathcal F_t]\|\\
        & \leq \left\| \E [G^0(x_t) - \nabla f^0(x_t)|\mathcal F_t] +  \sum_{i=1}^m \E \left[\eta G^i(x_t) \left(\frac{1}{\bar \alpha_t} - \frac{1}{\alpha_t} \right) + \eta( G^i(x_t) - \nabla f^i(x_t))  \frac{1}{\alpha_t}\bigg|\mathcal F_t\right] \right\| \\
        %   M_2(x_t) \left(\E [\|G^i(x_t)\|^2|\mathcal F_t] + \E [\|\alpha_t - \hat\alpha_t\|^2|\mathcal F_t] \right)\\
         & = \left\|\sum_{i=1}^m \E \left[\eta G^i(x_t) \left(\frac{1}{\bar \alpha_t} - \frac{1}{\alpha_t} \right) \bigg|\mathcal F_t\right] \right\| + b^0_t + \sum_{i=1}^m \frac{\eta}{\alpha_t^i}b^i_t
         \\ 
         & \leq   \sum_{i=1}^m \E \left[ \left\|\eta G^i(x_t) \left(\frac{1}{\bar \alpha_t^i} - \frac{1}{\alpha_t^i} \right)\right\| \bigg|\mathcal F_t\right] + b^0_t + \sum_{i=1}^m \frac{\eta}{\alpha_t^i}b^i_t
         \\
        & \leq  \sum_{i=1}^m  \sqrt{ \E [\eta^2\|G^i(x_t)\|^2|\mathcal F_t] \E \left[\frac{1}{(\bar\alpha_t^i)^4}\|\alpha_t^i - \bar\alpha_t^i\|^2\bigg|\mathcal F_t\right] } + b^0_t + \sum_{i=1}^m \frac{\eta}{\alpha_t^i}b^i_t\\
        & \leq \sum_{i=1}^m  \frac{\eta L^i \sigma_t}{(\alpha_t^i)^2}  + b^0_t + \sum_{i=1}^m \frac{\eta}{\alpha_t^i}b^i_t
       ,
    \end{align*}
\end{proof}

\subsubsection{Variance}\label{A:var}
\begin{proof}
    Indeed, by definition  $$v_t^2  := \E \|g_t - \E g_t \|_2^2  = \Var G^0(x_t) 
    + \eta^2 \sum_{i=1}^m
    \E\left\| \frac{G^i(x_t)-\E G^i(x_t)}{\bar\alpha_t^i} 
    + \E G^i(x_t)\left(\frac{1}{\bar\alpha_t^i} -\E\frac{1}{\bar\alpha_t^i}\right)\right\|^2_2.$$
    Therefore
     $$v_t^2 = \E_t   \|G^0(x_t,\xi_t) -  \nabla f^0(x_t)\|_2^2 
    + \eta\sum_{i=1}^m \E_t  \|G^i(x_t,\xi_t)\|_2^2\E_t\left(\frac{1 }{\bar \alpha_t^i} - \frac{1}{\alpha_t^i}\right)^2
    +  \eta\sum_{i=1}^m  \E_t \left(\frac{v_t^2}{\alpha_t^i} \right).$$
\end{proof}

\subsection{Proof of the adaptivity}\label{P1}
\begin{proof}
    For adaptivity, we require
    $$f^i(x_{t+1}) \leq \frac{f^i(x_{t})}{2}.$$
    Using $M^i$-smoothness, we can bound the $i$-th constraint growth:
    \begin{align*}
        f^i(x_{t+1})
        & \leq f^i(x_{t}) + \la \nabla f^i(x_t), x_{t+1} - x_t \ra + \frac{M^i}{2}\|x_t-x_{t+1}\|_2^2 \\
        &  = f^i(x_{t}) - \gamma_t \la \nabla f^i(x_t),g_t \ra + \gamma_t^2\frac{M^i}{2}\|g_t\|_2^2
        % \\
        % &\leq f^i(x_{t}) + \gamma_t \| \nabla f^i(x_t)\|_2\|g_t\|_2 + \gamma_t^2\frac{M^i}{2}\|g_t\|_2^2
    \end{align*}
    That is, the condition on $\gamma_t$ for adaptivity (and safety) we can formulate by
    $$ -\gamma_t \la \nabla f^i(x_t),g_t \ra + \gamma_t^2\frac{M^i}{2}\|g_t\|_2^2  \leq \frac{-f^i(x_{t})}{2} = \frac{\alpha_t^i}{2}.$$
    By carefully rewriting the above inequality without strengthening it, we get
    % Option one sims not the best
    %   \begin{align*}
    %     &     \gamma_t^2\frac{M^i}{2}\|g_t\|_2^2  - \gamma_t \la \nabla f^i(x_t),g_t \ra \pm  \frac{1}{2M^i}\|\nabla f^i(x_t)\|_2^2\leq \frac{\alpha_t}{2}\\
    %     & \frac{1}{2}\left\|\gamma_t\sqrt{M^i} g_t  -  \frac{\nabla f^i(x_t)}{\sqrt{M^i}}\right\|_2^2 \leq  \frac{1}{2M^i}\|\nabla f^i(x_t)\|_2^2 + \frac{\alpha_t}{2}\\
    %     & M^i\left\|\gamma_t g_t  -  \frac{\nabla f^i(x_t)}{M^i}\right\|_2^2 \leq  \frac{1}{M^i}\|\nabla f^i(x_t)\|_2^2 + \alpha_t\\
    %     & \left\|\gamma_t g_t  -  \frac{\nabla f^i(x_t)}{M^i}\right\|_2^2 \leq  \left\|\frac{\nabla f^i(x_t)}{M^i}\right\|_2^2 + \frac{\alpha_t}{M^i}\\
    %   \end{align*} 
    %   Option 2 more exact 
       \begin{align*}
        &     \gamma_t^2\frac{M^i}{2}\|g_t\|_2^2  - \gamma_t \la \nabla f^i(x_t),g_t \ra \pm  \frac{1}{2M^i}\frac{\la \nabla f^i(x_t),g_t\ra^2}{\|g_t\|_2^2}\leq \frac{\alpha_t}{2}
        \\
        & \left(\gamma_t\|g_t\|_2 - \frac{\la \nabla f^i(x_t),g_t\ra}{M_i\|g_t\|_2}\right)^2 
        \leq \frac{\alpha_t}{ M^i} + \frac{\la \nabla f^i(x_t),g_t\ra^2}{M_i^2\|g_t\|_2^2}
        \end{align*}
        Using the quadratic inequality solution, we obtain the following sufficient bound on the adaptive $\gamma_t:$ 
        $$ 
         \gamma_t\|g_t\|_2 
        \leq \frac{\la \nabla f^i(x_t),g_t\ra}{M_i\|g_t\|_2} + \sqrt{\frac{\alpha_t}{ M^i} + \frac{\la \nabla f^i(x_t),g_t\ra^2}{M_i^2\|g_t\|_2^2}} = (*)$$
        Then, we can rewrite this expression of the right part as follows:
        \begin{align*} 
          (*)& = \sqrt{\frac{\la \nabla f^i(x_t),g_t\ra^2}{M_i^2\|g_t\|_2^2} + \frac{\alpha^i_t}{ M^i} } + \frac{\la \nabla f^i(x_t),g_t\ra}{M_i\|g_t\|_2}
          = 
          \sqrt{\frac{\alpha_t^i}{ M^i}}
          \left(\sqrt{\frac{\la \nabla f^i(x_t),g_t\ra^2}{M_i \alpha_t^i\|g_t\|_2^2} + 1} + \frac{\la \nabla f^i(x_t),g_t\ra}{\sqrt{M_i \alpha_t^i}\|g_t\|_2}\right)\\
          &= \sqrt{\frac{\alpha_t^i}{ M^i}}
          \frac{1}{
          \sqrt{\frac{\la \nabla f^i(x_t),g_t\ra^2}{M_i \alpha_t^i\|g_t\|_2^2} + 1} - \frac{\la \nabla f^i(x_t),g_t\ra}{\sqrt{M_i \alpha_t^i}\|g_t\|_2}}
          = \frac{\alpha_t^i}{\sqrt{\frac{\la \nabla f^i(x_t),g_t\ra^2}{\|g_t\|_2^2} + M^i \alpha_t^i} - \frac{\la \nabla f^i(x_t),g_t\ra}{\|g_t\|_2}} =  \frac{\alpha_t^i}{\sqrt{(\theta_t^i)^2 + M^i \alpha_t^i} - \theta_t^i}
        \end{align*} 
Therefore, the condition $\gamma_t \leq  \min_{i\in[1,m]}\left\{\frac{\alpha_t^i}{\sqrt{(\theta_t^i)^2 + M^i \alpha_t^i} - \theta_t^i}\right\}
\frac{1}{\|g_t\|_2} $
is sufficient for $f^i(x_{t+1})\leq \frac{f^i(x_{t})}{2}.$ 
Using the Cauchy-Schwartz inequality, we can simplify this condition ( but making it  more conservative):
$$(*) \geq \frac{\alpha_t^i}{
          \sqrt{(\theta_t^i)^2 + \alpha_t M_i} +|\theta_t^i|}
          \geq 
         \frac{\alpha^i_t}{2|\theta_t^i| + \sqrt{\alpha_t^i M^i}}.$$
%Thus, the simpler condition $\gamma_t \leq  \min_{i\in[1,m]}\left\{\frac{\alpha^i_t}{2\frac{|\la \nabla f^i(x_t),g_t\ra|}{\|g_t\|_2} + \sqrt{\alpha_t^i M^i}}\right\}
%\frac{1}{\|g_t\|_2} $ is also sufficient for $f^i(x_{t+1})\leq \frac{f^i(x_{t})}{2}$ (but more conservative.) 
\end{proof}

\subsection{Proof of the local smoothness}\label{P2}

\begin{proof}
 Note that by definition of the log barrier, the hessian of it at the point $x_{t+1}$ is given by $$\nabla^2B_{\eta}(x_t) =  \nabla^2 f^0(x_{t+1}) + \sum_{i=1}^m \eta\frac{\nabla^2 f^i(x_{t+1})}{-f^i(x_{t+1})} + \sum_{i=1}^m \eta\frac{\nabla f^i(x_{t+1})\nabla f^i(x_{t+1})^T}{(-f^i(x_{t+1}))^2}.$$
 Based on that, 
\begin{align*}
    |\tilde g_t^T H_B(x_{t+1}) \tilde g_t| & \leq M^0\|\tilde g_t\|_2^2 + \eta \sum_{i=1}^m \frac{M^i}{\alpha_{t+1}^i}\|\tilde g_t\|_2^2 + \eta\sum_{i=1}^m  \frac{(\nabla f^i(x_{t+1})^T\tilde g_t/\|g_t\|_2)^2}{(\alpha_{t+1}^i)^2}\|\tilde g_t\|_2^2 \\
    & \leq \|\tilde g_t\|_2^2\left(M^0 + \eta \sum_{i=1}^m \frac{M^i}{\alpha_{t+1}^i} + \eta\sum_{i=1}^m  \frac{\la \nabla f^i(x_{t+1}), \tilde g_t\ra^2/\|\tilde g_t\|_2^2}{(\alpha_{t+1}^i)^2}\right)\\
    & \leq \|\tilde g_t\|_2^2\left(M^0 + 2\eta \sum_{i=1}^m \frac{ M^i}{\alpha_{t}^i} + 4 \eta\sum_{i=1}^m  \frac{\la \nabla f^i(x_{t+1}), \tilde g_t\ra^2}{(\alpha_{t}^i)^2 \|\tilde g_t\|_2^2}\right)
\end{align*}

Thus, $$M_2(x_t) = M^0 + 2\eta \sum_{i=1}^m \frac{ M^i}{\alpha_{t}^i} + 4 \eta\sum_{i=1}^m  \frac{\la \nabla f^i(x_{t+1}), \tilde g_t\ra^2}{\alpha_{t}^2 \|\tilde g_t\|_2^2}$$

$$M_2(x_t) \leq M^0 + 2\eta \sum_{i=1}^m \frac{ M^i}{\alpha_{t}} + 4 \eta\sum_{i=1}^m  \frac{4(\theta_t^i)^2 +(\theta_t^i)^2 + M^i\alpha_t^i + 2\theta_t^i\sqrt{M^i\alpha_t^i}}{(\alpha_{t}^i)^2 }$$
\end{proof}

\subsection{Proof of Keeping Distance Lemma \ref{lemma:keeping_distance} }\label{Appendix:keeping_distance}
Keeping distance is the key property, guaranteeing the regularity of the log barrier in the sense of a bounded norm, bounded smoothness and bounded variance. For the exact information case, without noise it is shown to converge without stating this property explicitly \citep{hinder2018one}. However, in the stochastic case this becomes crucial for stable convergence. At the same time, it helps to guarantee that the adaptive step sizes are not converging faster than $\frac{1}{t}$ asymptotically. This property follows from the fact that the step direction is the descent direction of the log barrier in expectation, together with the step size bounded by the smoothness of the log barrier. This guarantees that the method pushes the iterates $x_t$ away from the boundaries as soon as they come closer to them. We prove it in the following Lemma: 

When $\gamma_{t+1}=0$? When $-f^i(x_t)<c\eta.$

WE CAN PROVIDE THE ANALYSIS FOR THE MODEL-BASED APPROACH USING THE OPTIMISM AND PESSIMISM!
\begin{proof} 
 That implies that 
% \section{Proof of Lemma \ref{lemma:keeping_distance} }\label{Appendix:7}
%     \begin{proof} 
We first show that if $\alpha_t \geq 2c\eta_k$, then it holds that $\Prob\{\alpha_{t+1} \geq 2c\eta_k\}\geq 1-\frac{\de}{mT}$ (using the result of Lemma \ref{lemma:help}).

The possible values for $ \alpha_t^i$ (for $x_t\in \mathcal X$) can be split into the intervals: $0\leq 2c\eta_k\leq 4c\eta_k\leq \beta $, i.e., we have three cases:
 \begin{enumerate}
 \item[(1)] $\alpha_t^i\in [2c\eta_k, 4c\eta_k]$; 
 \item[(2)] $\alpha_t^i\in( 4c\eta_k,\beta]$; 
 \item[(3)] $\alpha_t^i\in(0,2c\eta_k).$ 
 \end{enumerate}
 
 \paragraph{Consider the first case (1) $\alpha_t^i\in [2c\eta_k, 4c\eta_k]$ for the iteration $t\in [T_k]$}.
 
 We show that with high probability $\alpha_{t+1}^i$ will not decrease $\Prob\{\alpha^i_{t+1} \geq 2c\eta_k|\alpha^i_{t} \geq 2c\eta_k\}\geq 1-\de.$ 
Using $M_i$-smoothness of $f^i(x)$ for all $ i \in [m]$, we get in conditional expectation
    \begin{align*} 
        \E_t f^i(x_{t+1})
        &
        \leq  f^i(x_t) + \E_t \la \nabla f^i(x_t),-\gamma_t g_t\ra + \E_t \frac{M^i}{2} \gamma_t^2\|g_t\|_2^2 
        \\
        &
        \leq  f^i(x_t) - \E_t \gamma_t\la \nabla f^i(x_t),
         \nabla B_{\eta_k}(x_t) + b_t\ra + \E_t \frac{M^i}{2} \gamma_t^2\|g_t\|_2^2.
    \end{align*}
What if for the LB gradient estimate we pick the "pessimistic" sample of model $F^i(x,\xi)$? This plays role in 1) adaptivity, 2) keeping distance. Then, what we get is:

    \begin{align*} 
        F^i(x_{t+1}, \xi_t)
        &
        \leq  F^i(x_t, \xi_t) +  \la \nabla F^i(x_t,\xi), -\gamma_t \tilde g_t\ra + \E_t \frac{M^i}{2} \gamma_t^2\|\tilde g_t\|_2^2 
        \\
        &
        \leq  F^i(x_t, \xi_t) - \gamma_t\la \nabla F^i(x_t, \xi_t),
         \nabla B_{\eta_k}(x_t, \xi_t)\ra + \E_t \frac{M^i}{2} \gamma_t^2\|\tilde g_t\|_2^2.
    \end{align*}

In particular, using this we can show that if $F^i(x_t) \leq -c\eta_t$, then during the next iteration it will decrease. What does this mean for $f^i(x_{t+1})$? Ideally, We would like to conclude that it will also be lower bounded. 
    
Next, note that
    $\la \nabla B^{\eta}(x_t,\xi_t), \nabla F^j(x_t,\xi_t)\ra =  \la\nabla F^0_{\nu_k}(x_t,\xi_t), \nabla F^j_{\nu_k}(x_t,\xi_t)\ra 
    + \sum_{i=1}^m\frac{\eta_k\la\nabla F^i(x_t,\xi_t), \nabla F^j(x_t,\xi_t)\ra}{-F^i(x_t,\xi_t)} 
    .$
Define the index set of $\eta_k$-active constraints by $I_t := \{i \in[m]
 :- F^i(x_t,\xi_t) \leq \eta_k\}$ and 
 recall \ref{fact:1}, then for all $F^i(x_t)\forall i\in I_t$ we get lower bound $\|\nabla F^i(x_t)\|_2\geq \frac{\beta-\eta_k}{R}.$ 
 Using  Assumption \ref{assumption:angles} and that $\eta_k\leq\eta_0\leq \beta/2$, we get $\|\nabla f^i_{\nu_k}(x_t)\|_2\geq \frac{\beta}{2R}.$ and 
    \begin{align}\label{eq:descent1}
        \la \nabla B^{\eta_k}(x_t,\xi_t), \nabla F^j(x_t, \xi_t)\ra 
        &\overset{\textcircled{\scriptsize 1}}{\geq} \frac{\eta_k}{2c\eta_k} \|\nabla f^j_{\nu_k}(x_t)\|^2_2 
        % \\
        % &
        + \sum_{i\in I_t}\frac{\eta_k}{-f^i_{\nu_k}(x_t)} \la\nabla f^i_{\nu_k}(x_t),\nabla f^j_{\nu_k}(x_t)\ra \nonumber
        \\
        & 
        -\|\nabla f^0_{\nu_k}(x_t)\|_2\|\nabla f^j_{\nu_k}(x_t)\|_2  
        - \sum_{i\notin I}\frac{\eta_k}{\beta/2} \|\nabla f^i_{\nu_k}(x_t)\|_2\|\nabla f^j_{\nu_k}(x_t)\|_2  \nonumber
        \\
        & 
        \overset{\textcircled{\scriptsize 2}}{\geq} \left(\left(\theta|I_t| + \frac{1}{2c}\right) \frac{\beta}{2R} - \frac{\eta_k}{\beta/2}m L\right)\|\nabla f^j_{\nu_k}(x_t)\|_2\nonumber
        \\
        & 
        \overset{\textcircled{\scriptsize 3}}{\geq} \left(\frac{\beta}{4cR} - m L\right)\|\nabla f^j_{\nu_k}(x_t)\|_2.
    \end{align}
 Hence, for $c
%  \leq \frac{\beta^2}{4mLR\eta_k} 
 \leq \frac{\beta}{4mLR} $ we have 
 \begin{align}\label{eq:descent}
 \la\nabla B^{\eta_k}_{\nu_k}(x_t),\nabla f^j_{\nu_k}(x_t)\ra\geq
%  \frac{2\tau_k}{\eta_k\sqrt{n_k}}
 \frac{\beta}{8cR}\|\nabla f^j_{\nu_k}(x_t)\|_2.
 \end{align}
 That is, we obtain the bound on increase of the value $f^i_{\nu_k}$: %(x_{t+1}) - f^i(x_t)$
% (Using $\hat M_2(x)\geq \frac{\sqrt{d}L}{\nu_k}\rightarrow \gamma_t \leq \frac{1}{\hat M_2(x)}\leq \frac{\nu_k}{\sqrt{d}L}$):
    \begin{align*}
        (\E_t f^i_{\nu_k}(x_{t+1}) - f^i_{\nu_k}(x_t)) &\leq - \gamma_t\la \nabla f^i_{\nu_k}(x_t),
         \nabla B^{\eta_k}_{\nu_k}(x_t)\ra
        % \\
        % &   
        + \gamma_t\|b_t\|_2 \| \nabla f^i_{\nu_k}(x_t)\|_2 + 
        % \gamma_t \frac{\sqrt{d}L}{\nu_k}\frac{\|g_t\|_2^2}{2\hat M_{2}(x_t)} 
        \gamma_t \frac{M^i}{2}\frac{\|g_t\|_2\hat\alpha_t}{2l} 
        % \|g_t\|_2\frac{\hat\alpha_t}{2L}
        % (\text{or }\frac{\sqrt{d}L\|g_t\|_2^2}{2\hat M_2(x)\nu_k})
        %  \\
        %  \\
        %  &
        % \leq \gamma_t\left(\frac{1}{2}\|g_t\|_2^2  - \frac{\tau_k}{\eta_k\sqrt{n_k}} \|\nabla f^i_{\nu_k}(x_t)\|_2\right).
    \end{align*}
 For the above, we can use $\|b_t\|_2 \leq b^0_t 
   + \eta \sum_{i=1}^m\E \frac{b^i_t}{\bar \alpha_t^i} \leq \nu M$  
%   $\Prob\{\|b_t\|_2\leq \frac{\tau_k}{\eta_k}\}\geq 1-\de$ 
   (for $\alpha_t^i\geq 2c\eta_k$ ).
%   and $n_k\geq \frac{\sigma^2}{c^2\eta_k^2}\ln\frac{Tm}{\de}$ according to Appendix \ref{Appendix:2}). 
 We also can get the following bound (using $\hat \alpha_t\geq c\eta_k$ and $v_t$)
    \begin{align}\label{eq:g_bound}
      \Prob\left\{\|g_t\|_2 \leq v_t + L\left(1+\frac{m}{c}\right)
    %   \left(L + \frac{\sigma\sqrt{\ln\frac{1}{\de}}}{\nu_k\sqrt{n_k}}\right)\left(1 + \frac{m}{c}\right)
      \right\}\geq 1-\de/Tm.
    \end{align} 
    Also, for this case $\hat\alpha_t\leq 4c\eta_k$.
Therefore, 
\begin{align*}
    \E_t f^i_{\nu_k}(x_{t+1}) - f^i_{\nu_k}(x_t)  &
         \leq \gamma_t\left(
         M^i\frac{4c^2\eta_k^2}{2l^2}
        %  \frac{(L(1+\frac{m}{c}) + \frac{\tau_k}{\eta_k\sqrt{n_k}})^2}{2(1+\frac{m}{c})} 
        %  \frac{\|\nabla f^i_{\nu_k}(x_t)\|_2}{c} 
        %  + \frac{\tau_k}{\eta_k\sqrt{n_k})^2}{2(1+\frac{m}{c})}
         + \left(
        %  2\frac{\tau_k}{\eta_k\sqrt{n_k}}
        %   \frac{\tau_k}{\eta_k\sqrt{n_k}}
        \nu \sum M^i
          -\frac{\beta}{8cR}\right) \frac{\|\nabla f^i_{\nu_k}(x_t)\|_2}{\|g_t\|_2^2}\right)\|g_t\|_2^2 \leq 0.
\end{align*}

    
% Hence, we can bound the increase of $f^i_{\nu_k}(x_t)$
%     \begin{align*}
%         &
%         f^i_{\nu_k}(x_{t+1}) - f^i_{\nu_k}(x_t)
%         % \\
%         % &
%         \leq \gamma_t\left(\frac{2c\sqrt{d}\eta_k}{\nu_k}\left(\frac{\tau_k}{\eta_k\sqrt{n_k}}+L(1+\frac{m}{c})\right)- 
%         % \frac{\tau_k}{\eta_k\sqrt{n_k}}
%         (mL-\frac{\tau_k}{\eta_k\sqrt{n_k}})
%         \frac{\beta}{2R}\right).
%     \end{align*}
Recall that $\nu_k\leq \frac{\eta_k}{2L}.$ 
Also, recall that $\|\nabla f^i_{\nu_k}(x_t)\|_2\geq \frac{\beta}{2R} $ and $ \frac{\beta}{2R}\geq 2cmL$ and the definition of $\tau_k.$ Hence, for $n_k\geq \frac{4\tau_k^2}{\eta_k^2L^2}$  with high probability we get
\begin{align*} 
        \E f^i_{\nu_k}(x_{t+1}) - f^i_{\nu_k}(x_t)   
        &   \leq 
        \gamma_t
        \Bigg(
        2\sqrt{d}Lc\left(\frac{L}{2}+L\left(1+\frac{m}{c}\right)\right)
        % \frac{\left(1.5+\frac{m}{c}\right)^2}{1+\frac{m}{c}}
        % \\
        % &
        + \frac{\beta}{2R}\left(\frac{L}{2} - \frac{\beta}{8cR}\right)\Bigg)
        \\
        & 
        \leq 
        \gamma_t
        \Bigg(2\sqrt{d}L^2(3c + 2m)
        - \frac{\beta^2}{16cR^2}\Bigg).
\end{align*}
That implies that in expectation $\sum_{t=1}^T \E (\hat \alpha_t^i)^2 \geq Tc\eta.$

Further, we use the properties of the martingales.

Using Azuma–Hoeffding inequality, noting that  $\sum_{t=1}^T [(\alpha_t^i)^2 -\E_t (\alpha_t^i)^2] $ is a martingale with respect to a filtration $\mathcal F_T$, we get 
$$\Prob\{\sum_{t=1}^T(\hat \alpha_t^i)^2  - \E \sum_{t=1}^T(\hat \alpha_t^i)^2 \geq \de\} \geq e^{\frac{-\de^2}{t\sum c^2}}$$
\begin{align}
   \sum_{t=1}^T \E(\hat \alpha_t^i)^2 = \sum_{t=1}^T ((\hat \alpha_t^i)^2 -(\E \hat \alpha_t^i)^2 ) + \sum_{t=1}^T (\E \hat \alpha_t^i)^2 \geq -\sqrt{T}\sigma^2 + Tc^2\eta^2.
\end{align}

% \begin{align*} 
%         \E f^i_{\nu_k}(x_{t+d}) - f^i_{\nu_k}(x_t)   
%         &   \leq 
%         \sum_{t=t}^{t+d}\gamma_t
%         \Bigg(
%         2\sqrt{d}Lc\left(\frac{L}{2}+L\left(1+\frac{m}{c}\right)\right)
%         % \frac{\left(1.5+\frac{m}{c}\right)^2}{1+\frac{m}{c}}
%         % \\
%         % &
%         + \frac{\beta}{2R}\left(\frac{L}{2} - \frac{\beta}{8cR}\right)\Bigg)
%         \\
%         & 
%         \leq 
%         \sum_{t=t}^{t+d} \gamma_t
%         \Bigg(2\sqrt{d}L^2(3c + 2m)
%         - \frac{\beta^2}{16cR^2}\Bigg).
% \end{align*}

The above directly implies that the constraint function does not decrease with high probability $\E f^i_{\nu_k}(x_{t+1}) - f^i_{\nu_k}(x_t) \leq 0$ for $c\leq \frac{\beta^2}{64 \sqrt{d} R^2L^2m}.$
 That is, for the first case we indeed have  $\Prob\{\alpha_{t+1}^i\geq 2c\eta_k | \alpha_{t}^i\geq 2c\eta_k \}\geq 1-\de/Tm.$
% Also, given that $\hat\alpha_t\geq c\eta_k$ and $\Prob\{f^i_{\nu_k}(x_t)\leq -\hat\alpha_t\}\geq 1-\de$, we can guarantee 
% % \begin{align}\label{eq:1}
%   $ \Prob\{f^i_{\nu_k}(x_t)\leq -c\eta_k\}\geq 1-\de.$
% \end{align}
% Combining it with the previous result, we get  
% $ \Prob\{f^i_{\nu_k}(x_{t+1})\leq -c\eta_k\}\geq 1-\de,$ that is $\hat\alpha_t \geq c\eta_k - \frac{\sigma}{\sqrt{n_k}}\sqrt{\ln\frac{1}{\de}}$. 

\paragraph{In the second case,} if $\alpha^i_t \geq 4c\eta_k$, we obtain for the next iteration $\Prob\{\alpha^i_{t+1} \geq 2c\eta_k|\alpha^i_t \geq 4c\eta_k\}\geq 1-\de/Tm,$ which brings us again to the first or second case. 
This implies that the result of Appendix  \ref{Appendix:2} holds for $t+1$th iteration.

% \paragraph{Continuing the same way,} we get that the cases (1) and (2), and the result of Appendix  \ref{Appendix:2} hold for all $x_t, t\in[T_k].$
\paragraph{Thus, using mathematical induction,} and carefully combining the conditional probabilities, if we start within cases (1) or (2), with high probability we never achieve the third case $\hat\alpha^i_t\leq \eta_k c,$ for all $x_t, t\in[T_k].$  The first and the second case correspond to the bound $\Prob\left\{\hat\alpha_t^i\geq c\eta_k, \forall t\right\}\geq 1-\de.$ Thus, both statements of Lemma \ref{lemma:keeping_distance} hold with probability $1-\de$.
% \end{proof}
% \input{lemma_9_proof_drafts}
% \input{lemma_9_new_proof}
\end{proof}


\subsection{Proof of Lemma \ref{lemma:convex_connection} for convex case }\label{A:3} 
\begin{proof}
\textbf{First step} By definition, the expressions for $B^{(k)}$ and $B^{(k+1)}$ are as follows
    \begin{align*}
        B^{(k)}(x) &= f^0(x) - \eta_k\sum_{i=1}^m\log (- f^i(x)) + \sum_{j=0}^k \frac{\mu_j}{2}\|x - \hat x_j\|^2\\
        B^{(k+1)}(x) & = f^0(x) - \eta_{k+1}\sum_{i=1}^m\log (- f^i(x)) + \sum_{j=0}^{k+1} \frac{\mu_{j}}{2}\|x - \hat x_j\|^2
    \end{align*}
    Then 
    \begin{align*}
        B^{(k+1)}(\hat x_{k+1}) - B^{(k)}(\hat x_{k+1}) & = (\eta_{k+1} - \eta_k) \sum_{i=1}^m-\log (- f^i(\hat x_{k+1})) +\mu_{k+1}\|\hat x_{k+1} - \hat x_{k+1}\|^2\\
        & = -\eta_{k+1}  \sum_{i=1}^m-\log (- f^i(\hat x_{k+1})) 
        % \\
        % & \leq \frac{\mu}{2}\|  \hat x_{k+1} - \hat x_{k}\|_2^2
    \end{align*} 
    % For having the second term negative, we need $-\log -f^i(x) >0$ that folds for $f^i(x) > -1.$ We can guarantee that by re-scaling. Currently we claim it using assumption. 
    % $$B^{(k)}(x_{k}^*) - B^{(k+1)}(x_{k+1}^*) \leq ?$$
    \textbf{Second step} By definition, $$B^{(k)}(x) = B^{(k+1)}(x) + (\eta_k - \eta_{k+1})\sum_{i=1}^m-\log-f^i(x) - \frac{\mu_{k+1}}{2}\|x -\hat x_{k+1} \|^2 $$
    Therefore, we can get the bound
    $$B^{(k)}(x_k^*) \leq B^{(k)}(x_{k+1}^*)= B^{(k+1)}(x_{k+1}^*) + (\eta_k - \eta_{k+1})\sum_{i=1}^m-\log(-f^i(x_{k+1}^*)) - \frac{\mu_{k+1}}{2} \| x_{k+1}^* -\hat x_{k} \|^2 $$
    Thus, 
    $$B^{(k)}(x_k^*) - B^{(k+1)}(x_{k+1}^*) \leq  \eta_{k+1}\sum_{i=1}^m-\log(-f^i(x_{k+1}^*)) - \frac{\mu_{k+1}}{2}\|\hat x_{k+1}^* -\hat x_{k} \|^2 $$
    % By definition of the optimum:
    % $$\nabla B^{(k+1)}(x_{k+1}^*)  = \nabla f^0(x_{k+1}^*) + \eta_{k+1}\sum_{i=1}^m\frac{\nabla f^i(x_{k+1}^*)}{-f^i(x_{k+1}^*)} +  \mu (\hat x_{k+1}^* -\hat x_{k+1}) = 0 $$ 
    % \begin{align*}
    % & \mu\|  \hat x_{k+1} - \hat x_{k}\|_2^2 + \mu\|  x_{k+1}^* - \hat x_{k}\|_2^2  - \mu\|  x_{k+1}^* - \hat x_{k+1}\|_2^2 \leq \mu\|  x_{k+1}^* - \hat x_{k}\|_2^2 + \mu\|  x_{k+1}^* - \hat x_{k}\|_2^2 \\
    % & = 2\mu\|  x_{k+1}^* - \hat x_{k}\|_2^2 \end{align*}
     \textbf{Third step}
    Combining the above together:
    \begin{align*}
        B^{(k+1)}(\hat x_{k+1}) - B^{(k+1)}(x_{k+1}^*)
        & = B^{(k)}(\hat x_{k+1})  -\eta_{k+1}  \sum_{i=1}^m-\log (- f^i(\hat x_{k+1}))  - B^{(k+1)}(x_{k+1}^*)\\
        & =  B^{(k)}(\hat x_{k+1}) - B^{(k)}(x_{k}^*)
        -\eta_{k+1}  \sum_{i=1}^m-\log (- f^i(\hat x_{k+1}))
        % \\
        % &
        + B^{(k)}(x_{k}^*) - B^{(k+1)}(x_{k+1}^*)\\
        & \leq B^{(k)}(\hat x_{k+1}) - B^{(k)}(x_{k}^*) + \eta_{k+1}  \sum_{i=1}^m-\log \frac{- f^i(x_{k+1}^*)}{- f^i(\hat x_{k+1})} -\frac{\mu_{k+1}}{2}\|  x_{k+1}^* - \hat x_{k}\|^2\\
        & \leq B^{(k)}(\hat x_{k+1}) - B^{(k)}(x_{k}^*) + O(\eta_{k+1})  -\frac{\mu_{k+1}}{2}\|  x_{k+1}^* - \hat x_{k}\|^2.
    \end{align*}
    Therefore 
    \begin{align*}
        \frac{\mu_{k+1}}{2}\|\hat x_{k+1} - x^*_{k+1}\|^2 
        & \leq \frac{M_2(\hat x_{k+1}) + \mu_{k+1}}{2}\|\hat x_{k+1} - x^*_{k}\|^2 + \eta_{k+1}  \sum_{i=1}^m-\log \frac{- f^i(x_{k+1}^*)}{- f^i(\hat x_{k+1})} -\frac{\mu_{k+1}}{2}\|  x_{k+1}^* - \hat x_{k}\|^2 \\
        & = \frac{M_2(\hat x_{k+1}) }{2}\|\hat x_{k+1} - x^*_{k}\|^2 +  \eta_{k+1}  \sum_{i=1}^m-\log \frac{- f^i(x_{k+1}^*)}{- f^i(\hat x_{k+1})}
    \end{align*}
    In the above the last inequality is due to the strong convexity.
\end{proof}

% \subsection{Simplified expression for $\gamma_t$}\label{A:gamma_simplified}
% [Write more carefully!]
% Indeed, as long as $\min \alpha_t^i\leq \frac{(\theta_t^i)^2}{L^0 + R}$
% \begin{align*}
%     \min_{i\in[m]}\left\{\frac{\alpha^i_t}{2|\theta^i_t| + \sqrt{\alpha_t^i M^i}}\right\}\frac{1}{\|\tilde g_t\|_2} 
%     & = 
%     \frac{\min_{i\in[m]}\left\{\frac{\alpha^i_t}{2|\theta^i_t| + \sqrt{\alpha_t^i M^i}}\right\}}{\la G^0(x_t,\xi_t) + \mu (x_t - x_0), \frac{\tilde g_t}{\|\tilde g_t\|_2}\ra + \eta \sum_{i=1}^m \frac{\la G^i(x_t,\xi_t), \frac{\tilde g_t}{\|\tilde g_t\|_2}\ra}{\bar\alpha_t^i}}
%     \\
%     & 
%     \geq 
%     \min_{i\in[m]}\left\{\frac{\alpha^i_t \bar\alpha_t^i}{m \eta(2|\theta^i_t| + \sqrt{\alpha_t^i M^i}) \la G^i(x_t,\xi_t), \frac{\tilde g_t}{\|\tilde g_t\|_2}\ra + \bar \alpha_t^i (G^0(x_t,\xi_t) + \mu (x_t - x_0)) } \right\} 
%     \\
%     & 
%     \geq 
%     \min_{i\in[m]}\left\{\frac{(\underline{\alpha}^i_t)^2}{m \eta(2|\theta^i_t| + \sqrt{\alpha_t^i M^i}) \bar \theta^i_t } \right\} 
%     % \\
%     % & 
%     \geq 
%     \min_{i\in[m]}\left\{\frac{(\underline{\alpha}^i_t)^2}{2m \eta(\hat \theta^i_t)^2 + \eta \hat  \theta^i_t  \sqrt{\alpha_t^i M^i}} \right\} 
% \end{align*}
% Recall that 
% \begin{align*}
%     \frac{1}{\hat M_2(x_t) + \mu} &
%     % =  \frac{1}{ M^0 + 2\eta \sum_{i=1}^m \frac{ M^i}{\hat \alpha_{t}} + 4 \eta\sum_{i=1}^m  \frac{4(\hat \theta_t^i)^2 +(\hat \theta_t^i)^2 + M^i\alpha_t^i + 2\theta_t^i\sqrt{M^i\alpha_t^i}}{(\hat \alpha_{t}^i)^2 }} 
%     % \\
%     % & 
%     \leq \min_{i\in [m]}\left\{\frac{(\alpha^i_{t})^2}{8 m\eta \hat\theta_t^i\sqrt{M^i\alpha_t^i} + 20 m\eta (\hat \theta^i_t)^2 + (\alpha^i_{t})^2(M_0 + \mu) }\right\}
% \end{align*}


% \subsection{Proof of lower bounds on $\sum \gamma_t$}\label{A:keeping_distance}
% % \begin{proof}
% \textcolor{red}{Not updated yet}
% \begin{lemma}\label{lemma:keeping_distance}
%     Under Assumptions \ref{assumption:1}, \ref{assumption:2_diameter}, \ref{assumption:3}, \ref{assumption:angles}, for all iterates $x_t$ of the \LBM algorithm during the single round $t\in[T_k]$ with $\eta_k < \beta/2$ the following holds for $\hat \alpha_t := \min_{i\in[1,m]} \{\hat\alpha_t^i\}$. 
%     % \begin{enumerate}
%     %     \item 
%         We have  
%         $\Prob\{  ~\hat\alpha_t\geq \eta_k c, \forall t\}\geq 1-\de$ for $n \geq \frac{\tau_k^2}{\eta^2_k}\ln(Tm)$,
%         with 
%         $c$ 
%         and $\tau_k$ defined in (\ref{eq:tau});
%     % \item $
%     %     \Prob\left\{ \|\zeta_t\|_2\leq \frac{\tau_k}{\eta_k\sqrt{n_k}}, \forall t\right\}\geq 1-\de.
%     % $
%     % \end{enumerate}
% \end{lemma}


\subsubsection{Lower bound on $\gamma_t$}\label{Appendix:5}
We get it by constructing bound on both of the terms inside the minimum.\\ 
%First, note that by definition $\hat M_{2}(x_t) = \frac{L}{\nu_k} + \eta_k  \sum _{i =1}^m\frac{\frac{L}{\nu_k}}{\hat\alpha_t^i}  + \eta_k \sum_{i=1}^m\frac{L}{(\hat\alpha_t^i)^2}.$ 
1) We have 
$\Prob\left\{\hat M_{2}(x_t) \leq \left(1+\frac{m}{c}\right)\frac{2\sqrt{d}L}{\nu_k}+4\frac{mL^2}{\eta_k c^2}\right\}\geq 1-\de$ (Due to Lemma \ref{lemma:keeping_distance}, and by definition of $\hat M_2(x_t)$), which implies 
    $$
        \Prob\left\{\frac{1}{\hat M_2(x_t)} \geq \eta_k\left(\frac{c^2}{4mL^2} + \frac{\nu_k}{ \eta_k}\frac{1}{(1+\frac{m}{c})\sqrt{d}L}\right)\right\}\geq 1-\de.
    $$
2) For $n\geq \frac{\sigma^2}{\nu_k^2}\ln \frac{1}{\de}$, using (\ref{eq:g_bound}) 
we get 
$\Prob\left\{\|g_t\|_2 \leq L \left(1.5 + \frac{m}{c}\right)\right\}\geq 1-\de.$
 Hence, we can bound $$\Prob\left\{\min_{i\in[1,m]}\frac{\hat\alpha_t^i}{2L^i\|g_t\|_2} \geq \frac{c\eta_k}{2L^2(1.5+\frac{m}{c})}\right\}\geq 1-\de.$$
 Therefore,
      $$
        \Prob\left\{\gamma_t \geq \frac{\eta_k}{2}\min 
        \left\{
        \frac{c^2}{4mL^2} + \frac{1}{(1+\frac{m}{c})\sqrt{d}L^2}, \frac{c}{L^2(1.5+\frac{m}{c})}\right\}
        \right\}\geq 1-\de,
    $$
    $$
        \Prob\left\{\gamma_t \geq \frac{\eta_k}{2L^2}\min 
        \left\{
        \frac{c^2}{4m} + \frac{c}{(1+\frac{m}{c})\sqrt{d}}, \frac{c}{1.5+m/c}\right\}
        \right\}\geq 1-\de.
    $$
Finally, 
    $$
        \Prob\left\{\gamma_t \geq \eta_k C 
        \right\}\geq 1-\de.
    $$
    with
    $$
    C := \frac{1}{2L^2}\min 
        \left\{
        \frac{c^2}{4m} + \frac{c}{\sqrt{d}(1+\frac{m}{c})}, \frac{c}{1.5+\frac{m}{c}}\right\}.
    $$

% \subsection{Proof of upper bounds on $\gamma_t$}\label{A:upper_bound_gamma} Using the Lemma \ref{lemma:LBGradEstimatorVarBias}  we upper bound the numerator part of this bound (\ref{eq:1}).
% % Our goal is now to use the inequality above to bound the left-hand-side in (\ref{eq2}) 
% First, recall that we 
% % $$\gamma_t = \min\left\{\min_{i\in[1,m]}\left\{\frac{\alpha^i_t}{2\hat\theta^i_t + \sqrt{\alpha_t^i M^i}}\right\}
% % \frac{1}{\|g_t\|_2} ,\frac{1}{M^0 + 6\eta \sum_{i=1}^m \frac{ M^i}{\alpha^i_{t}} + 20 \eta\sum_{i=1}^m  \frac{(\theta^i_t)^2}{(\alpha^i_{t})^2}}\right\},$$
% use $\hat\theta^i_t = \min\{l,|\theta^i_t|\}$ which is an upper bound on $|\theta^i_t|.$ Therefore, 
% \begin{align} \label{gamma_upper_bound}
% \gamma_t = \min\left\{\min_{i\in[1,m]}\left\{\frac{\hat\alpha^i_t}{2\hat\theta^i_t + \sqrt{\hat\alpha_t^i M^i}}\right\}
% \frac{1}{\|g_t\|_2} ,\frac{1}{M^0 + 6\eta \sum_{i=1}^m \frac{ M^i}{\hat\alpha^i_{t}} + 20 \eta\sum_{i=1}^m  \frac{(\theta^i_t)^2}{(\hat\alpha^i_{t})^2}}\right\} \leq \frac{(\hat\alpha_t^i)^2}{ml^2\eta}.
% \end{align}


% \end{proof}


